An Experimental Design Approach for Regret Minimization in Logistic Bandits

In this work we consider the problem of regret minimization for logistic bandits. The main challenge of logistic bandits is reducing the dependence on a potentially large problem dependent constant $\kappa$ that can at worst scale exponentially with the norm of the unknown parameter $\theta_{\ast}$. Abeille et al. (2021) have applied self-concordance of the logistic function to remove this worst-case dependence providing regret guarantees like $O(d\log^2(\kappa)\sqrt{\dot\mu T}\log(|\mathcal{X}|))$ where $d$ is the dimensionality, $T$ is the time horizon, and $\dot\mu$ is the variance of the best-arm. This work improves upon this bound in the fixed arm setting by employing an experimental design procedure that achieves a minimax regret of $O(\sqrt{d \dot\mu T\log(|\mathcal{X}|)})$. Our regret bound in fact takes a tighter instance (i.e., gap) dependent regret bound for the first time in logistic bandits. We also propose a new warmup sampling algorithm that can dramatically reduce the lower order term in the regret in general and prove that it can replace the lower order term dependency on $\kappa$ to $\log^2(\kappa)$ for some instances. Finally, we discuss the impact of the bias of the MLE on the logistic bandit problem, providing an example where $d^2$ lower order regret (cf., it is $d$ for linear bandits) may not be improved as long as the MLE is used and how bias-corrected estimators may be used to make it closer to $d$.

==> alg_glm2.tex <==
% !TeX root = main-file.tex
\section{Regret Minimization for Logistic Bandits}\label{sec:alg}

% \subsection{Experimental Design for Logistic Regression}

%\subsection{Problem Setting} % KJ: I felt this title has little role in understanding the paper.

%Let us formally define the problem.
%We assume access to a finite set of arms $\mc{X}\subset \mathbb{R}^d$. At each time $t\geq 1$ the learner chooses an arm $x_{I_t}\in \mc{X}$ and observes a Bernoulli reward $y_t\in \{0,1\}$ with 
%\[\mathbb{E}[y_t|x_{I_t}] = \mu(x_{I_t}^{\top}\theta)\]
%where $\mu(z) = \frac{1}{1+e^{-z}}$. Let $x^{\ast} = \arg\max_{x\in \mc{X}}x^\T \theta_{\ast}$, and without loss of generality we assume that $x^{\ast}$ is unique.
%The goal of the learner is to minimize the \emph{cumulative (pseudo-)regret} up to time $T$, that is,
%\[R_T = \sum_{t=1}^T \mu(x_{\ast}^{\top}\theta_{\ast}) - \mu(x_{I_t}^{\top}\theta_{\ast}).\]
Let us formally define the problem.
We assume access to a finite and fixed set of arms $\mc{X}\subset  \{x\in\mathbb{R}^d: \|x\|_2 \le 1 \}$. At each time $t\geq 1$ the learner chooses an arm $x_t\in \mc{X}$ and observes a Bernoulli reward $y_t\in \{0,1\}$ with 
\[\mathbb{E}[y_t|x_t] = \mu(x_t^{\top}\theta_*)~.\]
Let $x_* = \arg\max_{x\in \mc{X}}x^\T \theta_{\ast}$.
WLOG, we assume that $x_{\ast}$ is unique.
The goal of the learner is to minimize the \emph{cumulative (pseudo-)regret} up to time $T$:
$R_T := \sum_{t=1}^T \mu(x_{\ast}^{\top}\theta_{\ast}) - \mu(x_t^{\top}\theta_{\ast})$.

\textbf{Notations.} Let $ {\mc{F}_t}$ be the sigma algebra generated by the set of rewards and actions of the learner up to time $t$, i.e., $\sigma(x_1, y_1, \ldots, x_{t-1}, y_{t-1})$. 
We assume that the learner has knowledge of an upper bound $S$ on $\|\theta_{\ast}\|$. 
Define $ {\kappa} := \max_{\|x\|\leq 1} \mudot(x^\T \theta)^{-1}$ and $ {\kappa_0} := \max_{x\in \cX} \mudot(x^\T \theta)^{-1}$, the inverse of the smallest derivative of the link function among elements of $\mc{X}$. 
Denote by $ {\triangle_\cA}$ the set of probability distributions over the set $\cA$.
Let $\Supp(\lambda)$ with $\lambda \in \triangle_\cA$ be the subset of $\cA$ for which $\lambda$ assigns a nonzero probability.
We use $A\lsim B$ to denote $A$ is bounded by $B$ up to absolute constant factors.

%\subsection{Logistic Regression}

% \blake{Note for Lalit: Why is UCB a good idea? it is good from a regret standpoint but not a pulled an informative arm standpoint. Consider the 1d case. pulling the largest norm isn't the most optimal}

\textbf{Logistic Regression.}
We review logistic regression. %in the so-called fixed design setting.
Assume that we have chosen measurements $x_1, \ldots, x_t$ to obtain rewards $y_1,\ldots, y_t$. 
The \emph{maximum likelihood estimate} (MLE), $\hat{\theta}$ of $\theta_{\ast}$ is given by, 
\begin{align}\label{eq:mle}
    \hat{\theta} = \arg\max_{\theta\in \mR^d} \sum_{s=1}^t y_s\log(\mu(x_s^{\top}\theta))+(1-y_s)\log(1-\mu(x_s^{\top}\theta))
 \end{align}
% The MLE may not exist, but in our work such an event is rare and does affect our theoretical guarantees --
% if the nonexistence is still not desirable, one may first check if there exists a vector $\th$ such that $\sign(x_s^\T\th) = 2y_s - 1, \forall s\in[t]$ by forming a linear program, and if yes compute the MLE or otherwise compute a regularized version. \lalit{this is a bit vague - maybe we can move it to the appendix or punt on this issue?}
The Fisher information of the MLE estimator is  $H_t(\theta_{\ast}) := \sum_{s=1}^t \mudot(x_s^{\top}\theta_{\ast}) x_sx_s^{\top}$.
%  \begin{thm}[Theorem 1, \cite{jun2020improved}]\label{thm:concentration}
%   Let $\dt \le e^{-1}$. 
%   Let $\hat\th_t$ be the solution of Eq.~\eqref{eq:mle} where the $x_s$'s are a fixed design.
%   Fix $x\in\RR^d$ with $\|x\|\le1$. %\lalit{Do we need $|x_s|_2\leq 1$}\kj{good question; I will do this later}
%   %Let $t_{\mathsf{eff}}$ be the number of distinct vectors in $\{x_s\}_{s=1}^t$.
%   %Define ${\gamma(d)} \!=\! d + \log(6(2\!+\!\teff)/\dt)$.
%   Define the event $\cE_{\mathsf{var}} \!=\! \{\forall x', \fr{1}{\sqrt{2.2}}\,\|x'\|_{H_t(\th_*)^{-1}}
%   \!\le\! \|x'\|_{H_t(\hat\th_t)^{-1}} 
%   \!\le\! \sqrt{2.2}\, \|x'\|_{H_t(\th_*)^{-1}}\}$.
%   Then under the warmup condition \ref{eq:warmup} we have,
%   \begin{align*}
%     \PP\del{\!
%         |x^\T\!(\hat\theta_t\! -\! \theta_*)|  \!\le\! 3.5\|x \|_{\! H_{t} (\th_* \! )^{-\! 1}} 
%         \textstyle\!\sqrt{\log\fr{2(2+\teff)}{\dt}}
%         , \cE_{\mathsf{var}}
%     \!} \!\ge\! 1\!-\!\dt.
%   \end{align*}
% \end{thm}
%
% To appreciate this concentration result, consider that for the maximum likelihood estimator $\htheta_t$
% \begin{align*}
%     (\htheta - \theta_\ast)^\top x   \xrightarrow{D} \mc{N}\left(0, \|x\|_{H_t(\theta_\ast)^{-1}}^2\right)
% \end{align*}
% asymptotically as $t \rightarrow \infty$
% by the delta method. Hence, for large $t$ one may expect a confidence width of the form
% \begin{align*}
%     |(\htheta_t - \theta_\ast)^\top x| \lesssim \|x\|_{H_t(\theta_\ast)^{-1}}^2 \sqrt{2\log(1/\delta)}.
% \end{align*}
% as can be achieved via a Gaussian tail bound. Naturally, for small $t$ such concentration need not hold, but it is not immediately clear when one should expect CLT-like concentration.
% Theorem~\ref{thm:concentration} makes this precise and shows that if a warm up condition holds
% $\max_{s\in[t]} \|x_s\|^2_{H_{t}(\th_*)^{-1}} \le \fr{1}{\gamma(d)}$, then one enjoys concentration guarantees for $(\htheta_t - \theta_\ast)^\top x$ that are within a constant of the asymptotically optimal rate. 
%
Obtaining (near-)optimal regret hinges on the availability of tight confidence bounds on the \emph{means} of each arm. 
For technical reasons, tight confidence bounds (i.e., without extra factors such as $\sqrt{d}$ in the confidence bound like~\cite{faury2020improved}) require the data to observe the \textit{fixed design} setting: for each $s\in [t]$, $y_s$ is conditionally independent of $\{x_s\}_{s=1}^t\setminus \{x_s\}$ given $x_s$.
Recent work by \citet{jun2020improved} provide a tight finite-time fixed design confidence interval on the natural parameter of $x^\T \theta_\ast$ for any $x\in \mc{X}$. 
For regret minimization,  we instead require estimates of the mean parameter $\mu(x^\T \theta_\ast)$  each arm $x\in\cX$. 
Define ${\gamma(d)} \!:=\max\{\! d + \log(6(2\!+\!\teff)/\dt), 6.1^2\log(6(2\!+\!\teff)/\dt)\}$ where $t_{\eff}$ is the number of distinct vectors in $\{x_s\}_{s=1}^t$. We refer to the following assumption on our samples as the \emph{warmup condition}:
 \begin{equation}\label{eq:warmup}
      {\xi^2_t} := \max_{1\leq s\leq t} \|x_s\|^2_{H_{t}(\th_*)^{-1}} \le \fr{1}{\gamma(d)}~.
 \end{equation}
% \vspace{-em}
\begin{lem}\label{lem:mean_param_bound}
Fix $\delta \leq e^{-1}$. Let $\hat{\theta}_t$ denote the MLE estimate for a fixed design $\{x_1, \ldots, x_t\} \subset \cX$. Under the warmup condition~\eqref{eq:warmup}, with probability $1-\delta$, we have, $\forall x \in \cX$,
\begin{align} \label{eq:lem-mean_param_bound}
    &|x^\T(\hth_t - \th_*)| \le 1 \text{ and } 
    |\mu(x^\T\hat{\theta}_t) - \mu(x^\T{\theta}_\ast)| \\
    &\hspace{0.25cm}\leq 4.8\dot{\mu}(x^\T\theta_\ast)\|x\|_{H_t(\theta_\ast)^{-1}}\sqrt{\log(2(2 + t_\text{eff})|\cX|/\delta)}\nonumber. 
\end{align}
% Furthermore, for $|x^\T(\hat{\theta}_t - \theta_\ast)| \leq 1$, then the leading constant is $3.5e\leq 10$. 
\end{lem}
The proof relies on Theorem 1 of \cite{jun2020improved} and the (generalized) self-concordance of the logistic loss (\citet[Lemma 9]{faury2020improved}). %. \cite{bach2010self, faury2020improved}.
While similar results were used in the proof of SupLogistic in \citet{jun2020improved}, for our bandit algorithm below it is crucial to guarantee $\forall x\in\cX, |x^\T(\hth_t - \th_*)|\le 1$ as well.
As far as we know, this is the first non-trivial confidence bound on the mean parameter for logistic models. To contextualize this result, consider that via the delta-method, 
% \begin{align*}
$    \sqrt{t}(\mu(x^\T\htheta) - \mu(x^\T\theta_\ast))   \xrightarrow{D} \mc{N}\left(0, \dmu(x^\T\theta_\ast)^2\|x\|_{H_t(\theta_\ast)^{-1}}^2\right)$.
% \end{align*}
Hence, Lemma~\ref{lem:mean_param_bound} guarantees an asymptotically tight normal-type tail bound up to constant factors provided the warmup condition holds. 

% An advantage of our confidence width on the mean parameter is the scaling by $\dmu(\theta_\ast^\top x)$. Indeed, $\dmu(x) \approx e^{-x}$ for $x \geq 1$ making the confidence intervals far narrower. 



%%%%%%% moved to 2.4
% To operationalize this confidence interval for bandit algorithms we need to ensure that the warmup condition of the Lemma, namely, $\xi^2_t\leq \gamma(d)^{-1}$ is satisfied. For now, we will assume access to a generic warmup routine \texttt{BurnIn} that given a set of vectors $\mc{X}$
% samples arms in $\mc{X}$ in order to ensure that this condition holds. Algorithm 2 in \citep{jun2020improved} satisfies this condition, and we revisit the question of designing a warmup procedure in Section~\ref{sec:warmup}. Furthermore, we conjecture that the condition that $\xi^2_t\leq \gamma(d)^{-1}$ is unimprovable in general due to the inherent bias of the MLE and give a relevant example. 
% As we will see in the upcoming sections, the ability to estimate the mean of any arm allows us to constructed an improved regret minimization algorithm. 




\textbf{Experimental design.}
We leverage our tight confidence widths on the means $\mu(x^\T \theta_\ast)$ given in Lemma~\ref{lem:mean_param_bound} to develop a novel logistic bandit algorithm.
Motivated by the form of the confidence width on the mean parameter, we consider the following experimental design problem:
\begin{align*}
   {h^*} &:= \min_{\lambda\in \triangle_{\mc{X}}}\max_{x\in \mc{X}} \mudot(x^\T \theta_*)^2\|x\|_{H_{\lambda}(\theta_*)^{-1}}^2 \\
   &\text{~~ where ~~} H_{\lambda}(\theta) = \sum_{x\in \mc{X}} \lambda_x \mudot(x^\T \theta) xx^\T~,
\end{align*}
which we refer to as an \emph{$H$-optimal design}. 
That is, we want to find an allocation of samples over $\mc{X}$ minimizing the worst case confidence-width of Lemma~\ref{lem:mean_param_bound} for any $x\in \mc{X}$.
Note that $h^*$ depends on the arm set $\cX$, though we omit it for brevity.
This experimental design is closely linked to the $G$-optimal design objective for the MLE in an exponential family. Indeed, in our setting, the $G$-optimal design is 
\begin{align}\label{eq:g-optimal}
   {g^*} := \min_{\lambda\in\triangle_\cX} \max_{x\in \mc{X}} \|x\|^2_{H_\lambda(\theta_*)^{-1}}
\end{align}
% Hereafter, we use $h^*$ and $g^*$ instead of $h^*(\cX)$ and $g^*(\cX)$ when the dependence on $\cX$ is clear from context.
We point out that in the setting of linear bandits (i.e. the linear GLM), the celebrated Kiefer-Wolfowitz theorem states that the optimal value of this objective is just $d$  for any choice of $\mc{X}$ \cite{kiefer60theequivalence}. 
Hence, for any $\theta\in \mathbb{R}^d$, letting $\mc{Y} = \{\sqrt{\mudot(x^\T \theta)}x, x\in \mc{X}\}$ we see that
\begin{align*}
  h^*& = \min_{\lambda\in \triangle_{\mc{X}}}\max_{x\in \mc{X}} \mudot(x^\T \theta)^2\|x\|_{H(\theta_*)^{-1}}^2 \\
  &
  \leq \frac{1}{4} \min_{\lambda\in \triangle_{\mc{Y}}}\max_{y\in \mc{Y}} \|y\|^2_{(\sum_{y\in \mc{Y}} \lambda_y yy^{\top})^{-1}} 
  \leq \frac{d}{4}
\end{align*}
where we use $\mudot(z) \leq 1/4$ for the first inequality and the Kiefer-Wolfowitz theorem for the last inequality.
Since $\mudot(x^\T \theta)$ decays exponentially fast in $|x^\T \theta|$, this bound is overly pessimistic and in practice the values of the $H$-optimal will be much smaller.
In contrast, for the logistic setting, the $G$-optimal design objective may be large and we only have a naive bound $f_G(\mc{X})\leq \kappa_0 d$ obtained by naively lower bounding $H(\lambda) \geq \kappa_0\sum_{x\in \mc{X}} \lambda_x xx^\T $. In general these two criteria can produce extremely different designs. We provide an example where these designs are very different in our supplementary, see Figure~\ref{fig:exp_designs}.

Though experimental design for logistic models is an important and abundant topic, e.g., social science  applications where tight estimates on entries of $\theta$ are required for causal interpretation \cite{erlander05welfare}, as far as we know, the design above has not previously been proposed.
The closest that we are aware of is \citet{russell18design} that considers $\dmu(x^\T\th) \|x\|^2_{H(\th)^{-1}}$ rather than $\dmu(x^\T\th)^2 \|x\|^2_{H(\th)^{-1}}$. %, and a large body of literature focuses on the $D$-optimal design.
Most existing studies on optimal design in nonlinear models study theoretical properties of the design problem assuming the knowledge of $\th^*$ and then uses a plugin estimate.
However, they hardly study under what conditions the plugin estimate must satisfy for the plug-in design problem to closely approximate the true design problem and how one can efficiently collect data for the plugin estimate.
In contrast, we address these in our paper for the $H$- and $G$-optimal design problem for logistic models.
%Of course in practice, $\theta$ is not known and in general we use a plug-in estimator $\hat{\theta}$ to compute this design. We will see an example of this in the next section.

%\hspace{-.5em}
\subsection{From experimental design to regret minimization.}
%\hspace{-.5em}
%\subsection{H-Optimal Design Sampling Algorithm}
We now introduce our primary algorithm, \HOMER (\textbf{H}-\textbf{O}ptimal \textbf{ME}thod for \textbf{R}egret) which is centered around the $H$-optimal design objective and the confidence bound on the mean parameter given in Lemma~\ref{lem:mean_param_bound}. To build an initial estimate $\htheta_0$ of $\theta_\ast$, the algorithm begins by calling a warmup procedure \texttt{WarmUp} with the following guarantee: 

% \gray{
%   \begin{definition}
%     A warmup algorithm $\cA$ is said to be valid if:  Given a set $\cX$ and $\delta > 0$, at each time $t$ the algorithm $\cA$ pulls an arm $x_t$ to receive reward $y_t$. It terminates after $ {T_\delta}$ iterations and returns the MLE estimate $\htheta$ computed from $\{x_1, \cdots, x_{T_\delta}\}$ for a time step $T_\delta$ that satisfies 1) $T_\delta$ is measureable with respect to $\mc{F}_t$ \kj{$\cF_{T_\delta}$?} and 2) with probability at least $1-\dt$, the warmup condition \eqref{eq:warmup} holds.
% \end{definition}}
%\kj{}
%\kj{for the mathematical guarantee to work, we should let it return the arm pull assignments $\{N_x\}$ and then the bandit algorithm should pull it -- this way we can guarantee that it is a fixed design. I guess we could instead require that the warmup routine to satisfy the fixed design guarantee, but i feel the formal is a bit cleaner... below is my suggestion:}
%\kj{I attempted to have a shorter definition here.}
\begin{definition}
  A warmup algorithm $\cA$ is said to be $\dt$-valid if it returns an estimator $\hth_0$ such that it is certified to have $\PP(\forall x\in \cX: |x^\T(\hth_0 - \th_*)| \le 1 ) \ge 1-\dt$.
  %  sampling assignments $\{ {N_x} \in \cbr{0,1,2,\ldots} \}_{x\in\cX}$ such that when pulling arm $x$ exactly $N_x$ times the warmup condition \eqref{eq:warmup} holds.
\end{definition}
One natural attempt would the aforementioned experimental design approach of solving $ g^{\ast} = \min_{\lam \in \triangle_\cX } \max_{x\in\cX} \|x\|^2_{H_\lam (\th_*)^{-1}}  $.
We are guaranteed a solution $\lam^*$ with a support of at most $d(d+1)/2$ via Caratheodory's theorem; e.g., see~\citet[Theorem 21.1]{lattimore2020bandit}.
We can then pull arm $x$ exactly $\lceil \lam^*_x g^* \gamma(d)\rceil$ times to satisfy~\eqref{eq:warmup}, which in turns makes the MLE $\hth_0$ trained on these samples to perform a $\dt$-valid warmup.
However, we do not know $\th_*$.
Fortunately, when an upper bound $S$ on $\th_*$ is known, we can we consider the following naive warm-up procedure:
% We can guarantee the condition of~\eqref{eq:warmup} if an upper bound $S$  on $\th_*$ is known through the following warmup procedure:
\begin{align}\label{eq:warmup-naive}
  {g^{\naive}} =&  \min_{\lam\in\triangle_{\cX}} \max_{x\in\cX} \|x\|^2_{(H^\naive_\lam)^{-1}}  \nonumber\\
  & 
  \text{~~ where ~~}  {H^\naive_\lam} = \sum_x \lam_x \dmu(\|x\|S)x x^\T~.
\end{align}
%Given the solution $\hlam$ we can sample each arm $x\in\cX$ exactly $ {N_x^\naive} := \lcl \hlam_x  g^\naive(\hlam)\gam(d)\rcl$ times.
%
Let $\hat{\lambda}^{\naive}$ be the solution to this problem. Since $x^\T \th_* \le \|x\|\|\th_*\|$, we have $g^\naive \ge g^*$, so we can guarantee that the warmup condition~\eqref{eq:warmup} is satisfied when pulling each arm $x$ exactly  $\lceil \hat{\lambda}^{\naive}_x g^\naive \gamma(d)\rceil$ times.
Computing the MLE $\hth_0$ with these samples leads to a $\dt$-valid warmup with the sample complexity of $O(g^\naive\gam(d) + d^2)$ which in the worse case is  $O(\kappa d^2)$.
We discuss a more efficient warmup algorithm in Section~\ref{sec:warmup}; in this section, let us use this naive warmup procedure.

%Algorithm 2 from \citep[]{jun2020improved} as well as Algorithm \ref{alg:war} appearing later in Section~\ref{sec:warmup} both satisfy this definition.
% Using this initial estimate, the algorithm proceeds in rounds. 

The pesudocode of \HOMER can be found in Algorithm~\ref{alg:mix-exp-design-regret}.
In each round $k$, \HOMER maintains an active set of arms $\cX_k$ and computes two experimental design objectives over $\cX_k$, each using the MLE estimate from the previous round $\htheta_{k-1}$. The main experimental design, denoted $\lambda_k^H$,
is the H-optimal design in Line~\ref{line:H-opt} which ensures the gap $\mu(x_\ast^\T\theta_\ast) - \mu(x^\T \theta_\ast)$ is estimated to precision $2^{-k}$. This allows us to remove any arm $x$ whose gap is significantly larger than $2^{-k}$. 
The second optimal design, denoted $\lambda_k^G$,
is a G-Optimal design given in Line~\ref{line:G-opt}. It is necessary to ensure that the warmup condition holds in each round as samples are not shared across rounds. In order to trade off these two, possibly competing design criteria, \HOMER computes a mixture of $\lambda_k^H$ and $\lambda_k^G$ (denoted $\lambda_k$) with approximately $1-2^{-k}$ of the mass being given to the $H$-optimal design $\lambda_k^H$. 
Rather than sampling directly from this distribution
\HOMER relies on an efficient rounding procedure, \texttt{Round}. 
Given a distribution $\lambda$, tolerance $\epsilon$, and number of samples $n$, \texttt{Round} returns an allocation $\{x_i\}_{i=1}^n$ such that $H_n(\theta)$ is within a factor of $(1+\epsilon)$ $H(\lambda, \theta)$ for any $\theta \in \mathbb{R}^d$ provided $n \geq r(\epsilon)$ for a minimum number of samples $r(\epsilon)$. Efficient rounding procedures are discussed in \citet{fiez19sequential}. Recent work \citep[]{camilleri2021high} has shown how to avoid rounding for linear bandits through employing robust mean estimators, but it remains an open question for logistic bandits. 
\HOMER passes the mixed distribution to \texttt{Round} and samples according to the returned allocation to compute an MLE estimate $\htheta_k$. Finally it removes suboptimal arms using plug in estimates of their means $\mu(x^\T\htheta_k)$. 
% The algorithm begins with a warmup procedure that estimates the mean of each arm and $\hat{\theta}$ to sufficient precision to ensure the confidence widths in Lemma~\ref{lem:mean_param_bound}. Following the initial warmup, the algorithm initializes an active set of arms denoted $\mc{X}_k$ in the $k^\text{th}$ round. It computes an optimal design, leveraging the estimate $\htheta_{k-1}$ from the previous round. Then the algorithm eliminates arms it verifies to be suboptimal using Lemma~\ref{lem:mean_param_bound}. Indeed, the number of samples is chosen so as to ensure that with high probability $\mu(\theta_\ast^\top x_\ast) - \mu(\theta_\ast^\top x) \lesssim 2^{-k}$ for all $x \in \mc{X}_k$. By carefully selecting the number of samples to collect in each round, we ensure that the algorithm simultaneously suffers low regret in each round as all arms in the $k^\text{th}$ round are within $2^{-k}$ of the optima, while also removing suboptimal arms as the sampling proceeds. 

% In order to eliminate suboptimal arms, in each round the algorithm computes the objective $f_H(\mc{X}_k)$. The number of samples is proportional to $2^{2k}$ ensuring that the confidence widths shrink by $2^{-k}$ in each round. As a technical point, the algorithm also computes a $G$-Optimal design $f_G(\mc{X}_k)$ in each round in order to ensure the warmup conditional \ref{eq:warmup} of Lemma~\ref{lem:mean_param_bound} holds in every round. In contrast to a naive $G$-optimal design, however, in each round $k$ we are able to use the MLE estimate $\htheta_{k-1}$ from the preceding round. This allows us to optimally sample to ensure the warmup condition without need for the naive approximation that $H(\lambda) \leq \kappa_0 \sum_{x\in \mc{X}}xx^\top$. The designs $\lambda_H^k$ and $\lambda_G^k$ the optimize $f_H(\mc{X}_k)$ and $f_G(\mc{X}_k)$ respectively are mixed to form a single sampling distribution $\lambda_k$ with approximately $1 - 2^{-k}$ of the mass given to $\lambda_H^k$. In particular, as the algorithm proceeds the sampling distribution almost entirely follows the $H$-optimal design. Hence we refer to our algorithm as \HOMER: \textbf{H}-\textbf{O}ptimal \textbf{ME}thod for \textbf{R}egret and provide pseudocode in Algorithm~\ref{alg:mix-exp-design-regret}. \lalit{Can we write an expression for how much extra samples we take per phase? Is the idea that this gets swallowed by the other regret term? Really doubly logarithmic? We dont get a $\log(1/min_gap)$?}


% In the $k^\text{th}$ round, we wish to use the concentration result of Lemma~\ref{lem:mean_param_bound} to remove all arms $x$ such that $\mu(\theta_\ast^\top x_\ast) - \mu(\theta_\ast^\top x) > 2^{-k}$. Indeed, the $H$ optimal design minimizes the maximal confidence width on the estimated mean of any arm $x$-- $\mu(\htheta^\top x)$ using the maximum likelihood estimate $\htheta$. However, in order to apply the result of Lemma~\ref{lem:mean_param_bound}, we must ensure the warmup condition 
% $\max_{x\in \cX}\|x\|_{H_t(\theta_\ast)^{-1}}^2 \leq \cdot \gamma(d)^{-1}$ necessary for its correctness. To ensure this, we compute a second optimal design 
% % \[\min_\lambda \max_{} \]



% which uses successive rounds of G-optimal design to for regret minimization in logistic bandits. A downside of \texttt{RAGE-GLM} is that it removes

% \blake{This next bit needs to be moved down}

% In this section, we answer this question and actually achieve a tighter dependence on $d\dmu(x_\ast^\T\theta_\ast)$ than previous work, showing instead that that dependence is an artifact of past analysis and can be avoided through a tighter approach. To do so, we make use of Lemma~\ref{lem:mean_param_bound} and choose a design $\lambda$ that minimizes $\max_{x}\dmu(\theta_\ast^\Tx)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2$. This is equivalent to G-optimal design in the generalized linear setting, as we are minimizing the asymptotic variance of the estimate of $\mu(\theta_\ast^\Tx)$. As this design depends on the unknown $\theta_\ast$, in each round $k$, we use the maximum likelihood estimator $\htheta_{k-1}$ from the previous round. This allows us to optimize the confidence widths on all mean estimates simultaneously. A challenge in using the confidence width from Lemma~\ref{lem:mean_param_bound} is ensuring the condition $\max\|x\|_{H(\ast)^{-1}}^2 \lesssim \gamma(d)^{-1}$. Using past estimates $\htheta_{k-1}$ one can easily ensure this by computing the design $\lambda$ that minimizes $\max_{x}\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2$. However, this design may be suboptimal for minimizing $\max_{x}\dmu(\theta_\ast^\Tx)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2$. To trade off these objectives, we compute separate designs to optimize each objective and sample from a single mixed design weighted by the objective values of each optimization. We refer to the algorithm as \texttt{MDMA}: \textbf{M}ixed \textbf{D}esigns \textbf{M}ean-parameter \textbf{A}lgorithm and provide pseudocode in Algorithm~\ref{alg:mix-exp-design-regret}. 



% \blake{Add a note about rounding} - say recent work has been able to replace rounding with robust estimation. IT is still an open question on how to do this for logistic bandits. 

% \textfloatsep=.3em % this adjusts the space below algorithm.
\begin{algorithm}[t] \caption{\HOMER: H Optimal MEthod for Regret}
  \label{alg:mix-exp-design-regret}
  \small
  \begin{algorithmic}
    \Require{$\epsilon$, $\delta$, $\cX$, $\kappa_0$ }
    \State{$k=1, \cX_1 = \cX$, $\gamma(d, n, \delta) := \max\{d + \log(6(2+n)/\delta), 6.1^2\log(6(2+n)/\delta)\} $}
    \State {$\hat\theta_0\leftarrow$ \texttt{WarmUp}($\cX$)}  
    \While{$|\cX_k| > 1$ } 
    \State  $\delta_k = \delta/(4(2+|\cX|)|\cX|k^2)$
    \State{$\lambda_{k}^H = \arg\min_{\lambda\in \triangle_{\cX_k}} {\hat h_k(\lam)}$ \label{line:H-opt}}
    \State{\hspace{0.5cm}for ${\hat h_k(\lam)} := \max_{x\in\cX_k} \dot{\mu}(x^\T\hat{\theta}_{k-1})^2\|x\|_{H_\lambda(\hat{\theta}_{k-1})^{-1}}^2$}
    \State{$\lambda_{k}^G = \arg\min_{\lambda\in \triangle_{\cX_k}} \del{ {\hat g_k(\lambda)}:=
        \max_{x\in\cX_k} \|x\|_{H_\lambda(\hat{\theta}_{k-1})^{-1}}^2} $\label{line:G-opt}} 
    \State{$n_k^H = \lceil 6(1+\epsilon)6.1^2 3^3 2^{2k} \hat h_k(\lam_k^H)\log(\delta_k^{-1}) \rceil$}
    \State{$n_k^G = \lceil 6(1+\epsilon)\gamma(d, |\cX_k|, \delta_k) \hat g_k(\lam_k^G) \rceil$}
    \State{$\Tilde{\lambda}_{k,i} = \max\left\{\frac{n_k^H}{n_k^H + n_k^G}\lambda_{k,i}^H, \frac{n_k^G}{n_k^G + n_k^H}\lambda_{k,i}^G \right\}, \forall i\in[n], $}
    \State{\hspace{0.5cm}where $\lambda_{k,i}^H$ and $\lambda_{k,i}^G$ are the $i$-th entry of $\lambda_k^H$ and $\lambda_k^G$}
    \State{$\lambda_{k,i} = \Tilde{\lambda}_{k,i} /\sum_{j=1}^n\Tilde{\lambda}_{k,j}$ and $n_k = \max\{n_k^H + n_k^G, r(\epsilon)\}$}
    \State{$x_1, \ldots, x_{n_k} \larrow \texttt{Round}( n_k, \lambda_k, \epsilon) $} 
    \State{Observe $y_1, \cdots, y_{n_k}$, compute MLE $\hat\theta_k$ with $ \{(x_i,y_i)\}_{i=1}^{n_k}$. }
    % \State{$\cX_{k+1}\leftarrow \cX_k \setminus \left\{x\in \cX_k:\max_{x'\in \cX_k}\mu(x'^\T\hat{\theta}_k) - \mu(x^\T\hat{\theta}_k) \geq 2\cdot 2^{-k}\right\}$}
    \State{$\cX_{k+1}\leftarrow \cX_k \setminus \left\{x\in \cX_k:\underset{x'\in \cX_k}\max\mu(x'^\T\hat{\theta}_k) - \mu(x^\T\hat{\theta}_k) \geq 2\!\cdot \!2^{-k}\right\}$}
    \State{$k\gets k+1$}
    \EndWhile
    \State Continue to play the unique arm in $\mc{X}_k$ for all time.
  \end{algorithmic}
\end{algorithm}

%\hspace{-.5em}
% \subsection{Theoretical Guarantees}
\textbf{Theoretical Guarantees.}
We now present theoretical guarantees of \HOMER.
%\hspace{-.5em}
% \begin{thm}\label{thm:mix_regret_complexity}
% Fix $\delta \leq e^{-1}$ and suppose there is a generic warmup algorithm takes $T_B = o(d^2/\kappa\log(|\cX|/\delta))$ samples and satisfies the conditions of Lemma~\ref{lem:mean_param_bound}. 
% Define $T' := T - T_B$ to be the samples and assume $T' > 0$. Define $\cS_t = \{x \in \cX: \mu(x_\ast^\T\theta_\ast) - \mu(\theta_\ast^\Tx) \leq 2^{-k}\}$. 
% With probability at least $1-\delta$, 
% algorithm~\ref{alg:mix-exp-design-regret}, for any $\nu > 0$ obtains a regret within a doubly logarithmic factor of
% \begin{align*}
%     d^2/\kappa\log(|\cX|/\delta) & + T'\nu + \lceil\log_2((\Delta \vee \nu)^{-1})\rceil r(\epsilon) + (1+\epsilon)\gamma(d, |\cX|, \delta) \min_\lambda\max_{x\in\cX} \|x\|_{H(\lambda, {\theta}_{\ast})^{-1}}^2 
%     \\ &  + (1+\epsilon)
%     \log\left(\frac{|\cX|}{\delta}\right)\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} \min_\lambda\max_{x\in\cS_k} \frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x \vee \nu}
% \end{align*}
% Minimizing $\nu$, we achieve a minimax regret of 
% \begin{align*}
%     \widetilde{O}\left(\sqrt{T\min_\lambda\max_{x}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\log(|X|/\delta)}  + d^2/\kappa\log(|\cX|/\delta)\right).
% \end{align*}
% Additionally, setting $\nu = 0$, Algorithm \ref{alg:mix-exp-design-regret} achieves an instance dependent regret of 
% \begin{align*}
%     \widetilde{O}\left(\min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta)  + \frac{d^2}{\kappa}\log(|\cX|/\delta)\right)
% \end{align*}
% where $\widetilde{O}$ hides constants and doubly logarithmic factors. 
% \end{thm}
%
%
%
% \begin{thm}\label{thm:mix_regret_complexity}
% Fix $\delta \leq e^{-1}$ and suppose there is a generic warmup algorithm that incurs regret $R_{B}$, takes $T_B$ samples, and returns a $\hat{\theta}$ that satisfies the conditions of Lemma~\ref{lem:mean_param_bound}. 
% Define $T' := T - T_B$ and assume $T' > 0$. %Define $\cS_t = \{x \in \cX: \mu(x_\ast^\T\theta_\ast) - \mu(\theta_\ast^\Tx) \leq 2^{-k}\}$. 
% With probability at least $1-\delta$, 
% algorithm~\ref{alg:mix-exp-design-regret}, obtains a regret within a doubly logarithmic factor of
% \begin{align*}
%   c_1\min\left\{\sqrt{T\min_\lambda\max_{x}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\log(|X|/\delta)},  \min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta)\right\} + c_2\frac{d^2}{\kappa}\log(|\cX|/\delta).
% \end{align*}
% for $c_1, c_2$ absolute constants. \kj{we could define those two min max quantity separately so we can make it into the linewidth}
% % Additionally, Algorithm \ref{alg:mix-exp-design-regret} achieves an instance dependent regret of 
% % \begin{align*}
% %     \widetilde{O}\left(\min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta)  + \frac{d^2}{\kappa}\log(|\cX|/\delta)\right)
% % \end{align*}
% % where $\widetilde{O}$ hides constants and doubly logarithmic factors. 
% \end{thm}
% \begin{thm}\label{thm:mix_regret_complexity}
%   Fix $\delta \leq e^{-1}$ and suppose \texttt{WarmUp} draws at most $T_B$ samples and incurs regret at most $R_B$. 
%   Define $ {T'} := T - T_B$ and assume $T' > 0$.
%   % Finally, define 
%   % \[\rho^H(\theta_\ast) = \min_{\lambda \in \Delta_{\cX}}\max_{x \in \cX}\dot{\mu}(x^\T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 \ \text{ and } \ \rho^G(\theta_\ast) = \min_{\lambda \in \Delta_{\cX}}\max_{x \in \cX}\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\]
%   With probability at least $1-2\delta$, 
%   algorithm~\ref{alg:mix-exp-design-regret}, obtains a regret within a doubly logarithmic factor of 
%   \begin{align*}
%     \min\left\{\sqrt{h^* T}, \frac{h^*}{\Delta}\right\}\log(|X|/\delta) + \gamma(d) g^* + r(\epsilon)\log\left(\sqrt{T/h^*} \wedge \Delta^{-1}\right) + R_B.
%   \end{align*}
%   where $\Delta := \min_{x\in \mc{X} \sm \{x_*\}} \mu(x_{\ast}^{\top} \theta_{\ast}) - \mu(x^\T  \theta_*)$. 
  
%   %\{\mu(x_\ast^\T\theta_\ast) -  \mu(x^\T\theta_\ast) | \mu(x_\ast^\T\theta_\ast) -  \mu(x^\T\theta_\ast) > 0\}$. 
%   % \lalit{Os}
%   % \begin{align*}
%   %   c_1\sqrt{T\min_\lambda\max_{x}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\log(|X|/\delta)} + R_B.
%   % \end{align*}
%   % and 
%   % \begin{align*}
%   %   c_2 \min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta) + R_B.
%   % \end{align*}
%   % for $c_1, c_2$ absolute constants. 
% \end{thm}
% T

\begin{thm}\label{thm:mix_regret_complexity}

  Fix $\delta \leq e^{-1}$ and suppose \texttt{WarmUp} draws at most $T_B$ samples and incurs regret at most $R_B$. 
  Define $ {T'} := T - T_B$ and assume $T' > 0$.
  Choose a rounding procedure with $r(\eps) = O(d/\eps^2)$  (e.g., \citet[Appendix B]{fiez19sequential}) and set $\eps = O(1)$.
  Let $\Delta := \min_{x\in \mc{X} \sm \{x_*\}} \mu(x_{\ast}^{\top} \theta_{\ast}) - \mu(x^\T  \theta_*)$
  Then, with probability at least $1-2\delta$, 
  \HOMER obtains a regret within a doubly logarithmic factor of 
  \begin{align*}
    R_{B} &+ \min_{\nu\geq 0} \del{ T \nu + \frac{d \dmu(x_*^\T\th_*)}{\Delta \vee \nu} \ln\del{\fr{|\cX|}{\dt}} + d\ln\del{\frac{1}{\Delta \vee \nu}} } \\
    &+ d\kappa_0\del{d + \ln\del{\frac{|\cX|}{\dt}}}~.
    % \min\left\{\sqrt{d \dot\mu(x_{\ast}^{\top}\theta_{\ast}) T}, \frac{d \dot\mu(x_{\ast}^{\top}\theta_{\ast})}{\Delta}\right\}\log(|\cX|/\delta) + (1+r(\epsilon))\log(\Delta^{-1}) + d\gamma(d)\kappa_0 + R_B.
  \end{align*}
%   \kj{shouldn't we have $\sqrt{\log(|\cX|/\dt)}$ for the $\sqrt{T}$ regret?}
%   where $\Delta := \min_{x\in \mc{X} \sm \{x_*\}} \mu(x_{\ast}^{\top} \theta_{\ast}) - \mu(x^\T  \theta_*)$. 
  %\{\mu(x_\ast^\T\theta_\ast) -  \mu(x^\T\theta_\ast) | \mu(x_\ast^\T\theta_\ast) -  \mu(x^\T\theta_\ast) > 0\}$. 
  % \lalit{Os}
  % \begin{align*}
  %   c_1\sqrt{T\min_\lambda\max_{x}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\log(|X|/\delta)} + R_B.
  % \end{align*}
  % and 
  % \begin{align*}
  %   c_2 \min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta) + R_B.
  % \end{align*}
  % for $c_1, c_2$ absolute constants. 
\end{thm}
% 

\begin{remark}
Using the naive warmup~\eqref{eq:warmup-naive}, the one can show that $R_B = O\left(d^2\kappa\log(|\cX|/\delta)\right)$.
\end{remark}
%A key distinction of this bound is that we can even achieve a \emph{dimension independent} regret for the leading term $\ln(1/\dt)$ for some cases. 
%Indeed, consider a `polarized' setting where the mean of every arm is either very large or very small such that $\dmu(x^\T\theta_\ast) \leq 1/d$ for all $x$. In this setting, the Kiefer-Wolfowitz theorem implies that our main term is bounded by $\sqrt{T}$ independent of $d$ and the regret is instead dominated by the warm up.

% Furthermore, this is the first instance-dependent regret guarantee that we are aware of for logistic bandits. The form of our instance dependent regret bound matches similar quantities known for linear bandits such as Theorem 2.3 of \citep{foster2020instance}. \lalit{Can this be cut?}

% \begin{thm}\label{thm:mix_regret_complexity}
% Fix $\delta \leq e^{-1}$ and suppose there is a generic warmup algorithm takes $T_B = o(d^2/\kappa\log(|\cX|/\delta))$ samples and satisfies the conditions of Lemma~\ref{lem:mean_param_bound}. 
% Define $T' := T - T_B$ to be the samples and assume $T' > 0$. Define $\cS_t = \{x \in \cX: \mu(x_\ast^\T\theta_\ast) - \mu(\theta_\ast^\Tx) \leq 2^{-k}\}$. 
% With probability at least $1-\delta$, 
% algorithm~\ref{alg:mix-exp-design-regret}, obtains a regret within a doubly logarithmic factor of
% \begin{align*}
%   c_1\min\left\{\sqrt{T\min_\lambda\max_{x}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\log(|X|/\delta)},  \min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta)\right\} + c_2\frac{d^2}{\kappa}\log(|\cX|/\delta).
% \end{align*}
% for $c_1, c_2$ absolute constants. \kj{we could define those two min max quantity separately so we can make it into the linewidth}
% % Additionally, Algorithm \ref{alg:mix-exp-design-regret} achieves an instance dependent regret of 
% % \begin{align*}
% %     \widetilde{O}\left(\min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta)  + \frac{d^2}{\kappa}\log(|\cX|/\delta)\right)
% % \end{align*}
% % where $\widetilde{O}$ hides constants and doubly logarithmic factors. 
% \end{thm}
% % This result 

% \begin{thm}\label{thm:mix_regret_complexity}
% Fix $\delta \leq e^{-1}$ and suppose there is a generic warmup algorithm takes $T_B = o(d^2/\kappa\log(|\cX|/\delta))$ samples and satisfies the conditions of Lemma~\ref{lem:mean_param_bound}. 
% Define $T' := T - T_B$ to be the samples and assume $T' > 0$. Define $\cS_t = \{x \in \cX: \mu(x_\ast^\T\theta_\ast) - \mu(\theta_\ast^\Tx) \leq 2^{-k}\}$. 
% With probability at least $1-\delta$, 
% algorithm~\ref{alg:mix-exp-design-regret}, obtains a regret within a doubly logarithmic factor of
% \begin{align*}
%     \widetilde{O}\left(\sqrt{T\min_\lambda\max_{x}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\log(|X|/\delta)}  + d^2/\kappa\log(|\cX|/\delta)\right).
% \end{align*}
% Additionally, Algorithm \ref{alg:mix-exp-design-regret} achieves an instance dependent regret of 
% \begin{align*}
%     \widetilde{O}\left(\min_{\lambda \in \Delta_{\cX}}\max_{x\in \cX}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta)  + \frac{d^2}{\kappa}\log(|\cX|/\delta)\right)
% \end{align*}
% where $\widetilde{O}$ hides constants and doubly logarithmic factors. 
% \end{thm}


% Recently, \citet{abeille2021instance} proposed an optimistic UCB style algorithm called OFULog, establishing a regret bound of $\tilde O(d\ln^2(\kappa)\sqrt{\mudot(x_{\ast}^{\top}\theta_{\ast})T} + d^2\kappa)$ in the fixed arm-set setting which shows an additive dependence on $\kappa$ instead of a multiplicative dependence.\footnote{
%     In the case where there are few sub-optimal arms, they improve this additive dependence to a term that at worse could scale with the number of arms without the factor $\kappa$.
% } In the finite armed contextual bandit setting, \citet{jun2020improved} propose an improved fixed design confidence interval and adapted a SupLinRel style algorithm \cite{auer02finite} called SupLogistic to establish a regret scaling like $\tilde{O}(\sqrt{dT} + \kappa^2 d^3)$.\footnote{
%     \citet{jun2020improved} in fact have reported that the lower order term is $O(\kappa^2 d)$, but there is a hidden dependency on $d$.
%     This is because they assume that the expected minimum eigenvalue is at least $\sig_0^2$, but $\sig_0^2$ is $1/d$ at best. Our reported rate is for the best case of $\sig_0^2 = 1/d$.
% }
% To compare the leading term of the regret bound, SupLogistic achieves a better dependence on $d$ and $\kappa$.
% However, it has a worse dependence with $\dmu(x_*^\T\th_*)$ due to the changing arm set setting and makes a strong assumptions of stochastic contexts and bounded minimum eigenvalues.
% The regret bound of OFULog is free of these assumptions and have a better lower-order terms, but the leading term is suboptimal.
% We discuss more on related work in the appendix.
The \texttt{OFULog} algorithm of
\citep{abeille2021instance} achieves a regret bound of $\tilde O(d\ln^2(\kappa)\sqrt{\mudot(x_{\ast}^{\top}\theta_{\ast})T} + d^2\kappa)$ where the lower order term may be improved for the case where there are few sub-optimal arms so the lower order term scales with the number of arms without the factor $\kappa$. 
    % In the case where there are few sub-optimal arms, they improve this additive dependence to a term that at worse could scale with the number of arms without the factor $\kappa$.
\texttt{SupLogistic} of \citet{jun2020improved} follows SupLinRel-type sampling scheme to eliminates arms based on their natural parameter estimates and achieves a regret of $\tilde{O}(\sqrt{dT} + \kappa^2 d^3)$.\footnote{
    \citet{jun2020improved} in fact have reported that the lower order term is $O(\kappa^2 d)$, but there is a hidden dependency on $d$.
    This is because they assume that the expected minimum eigenvalue is at least $\sig_0^2$, but $\sig_0^2$ is $1/d$ at best. Our reported rate is for the best case of $\sig_0^2 = 1/d$.
}
% While the leading term of SupLogistic regret improves upon that of \citet{abeille2021instance} except for $\dmu(x_\ast^\T\theta_\ast)$, .
To compare the leading term of the regret bound, SupLogistic achieves a better dependence on $d$ and $\kappa$.
However, it has a worse dependence with $\dmu(x_*^\T\th_*)$ due to the changing arm set setting and makes strong assumptions of stochastic contexts and bounded minimum eigenvalues.
The regret bound of OFULog is free of these assumptions and have a better lower-order terms, but the leading term is suboptimal.

In the following Corollary, we further upper bound the result of Theorem~\ref{thm:mix_regret_complexity} in order to compare to the results of \citep[]{abeille2021instance} and \citep{jun2020improved} and show that \HOMER enjoys state of the art dependence on $d$, $\dmu(x_\ast^\T\theta_\ast)$, and $\log(\kappa)$ simultaneously and also matches the state-of-the-art worst-case lower order terms $d^2\kappa$. % in the worst case. 
\begin{cor}\label{cor:minimax_regret}
  Suppose we run \HOMER with $\dt = 1/T$ with the naive warmup~\eqref{eq:warmup-naive}  in the same setting as Theorem~\ref{thm:mix_regret_complexity}.
  Then, \HOMER satisfies 
  \begin{align*}
    \EE[R_T] = &\hat O\left(\left(  \sqrt{dT\dmu(x_\ast^\T\theta_\ast)\log(|\cX|T)} \right.\right. \\
    &\hspace{0.75cm} \left.\left.\wedge \frac{d \dmu(x_*^\T\theta_*) \log(|\cX| T)}{\Delta}  \right) + d^2\kappa \log(|\cX|T) \right)
  \end{align*}
  where $\hat O$ hides doubly logarithmic factors.
\end{cor}

This highlights that \HOMER simultaneously enjoys the optimal dependence on $d$ exhibited by \texttt{SupLogistic} and the state of the art dependence on $\dmu(x_\ast^\T\theta_\ast)$ seen in \texttt{OFULog}. Furthermore, \HOMER avoids a dependence on $\log(\kappa)$ in its leading term. 
% {\color{blue} We stress however, that the scaling $d\dmu(x_\ast^\T\theta_\ast)$ is introduced only as an upper bound on the result of Theorem~\ref{thm:mix_regret_complexity}. In general, a dependence of $d\dmu(x_\ast^\T\theta_\ast)$ on regret guarantees exhibited in past work may be more an artifact of past analyses than a fundamental quantity in logistic bandits. }

% In contrast to previous works, a key distinction of our method is that it avoids an explicit dependence on $d$ in the leading term. While the Kiefer-Wolfowitz theorem allows one to bound the $H$-Optimal design objective by $d/4$, we stress that the true value can be mush smaller as $\dmu(z)$ decreases exponentially. Furthermore, we avoid a dependence on $\|\theta_\ast\|^2$ in the leading term. Moreover, this is the first instance dependent regret bound that we are aware of for logistic bandits.  
% \lalit{Can we give an example where we are actually dimension independent on the main term? For example if $\max_{x}\mudot(x^\T \theta)\leq 1/d$. This seems like a real contribution? So in that case all the regret comes from warmup. Now past-work shows that }

% As an interpretation of this, one may consider the special case where $x_i = e_i$ and this problem reduces to the case of standard multiarmed bandits. In this setting, the leading term $\min_\lambda \max_{x}$ is $O\left(\sum_{i=2}^n\frac{1}{\Delta_i}\right)$ up to logarithmic factors matching optimal instance dependent rates for regret as in \cite{lattimore17theend}.
% \lalit{Not really? This doesn't have variances or KL's?}
% Additionally, our regret bounds both avoid the dependence on $d\dmu(x_\ast^\T\theta_\ast)$ as appeared in the result of \cite{abeille2021instance}. As $\dmu(x_\ast^\T\theta_\ast)$ is generally a small quantity, one may reasonably wonder how our bound compares to this rate and whether a dependence on $d\dmu(x_\ast^\T\theta_\ast)$ is fundamental for logistic bandits or is an artifact of past analyses. In the corollary below, we argue in favor of the latter and show that our regret bound can be further bounded in terms of this quantity



% Note that our minimax regret bound does not explicitly depend on $d$ or $\dmu(x_\ast^\T\theta_\ast)$ in the leading term, in contrast to the result of \cite{abeille2021instance}. In fact, we may further upper bound our regret guarantee to demonstrate improved dependence on both of these factors as well as improved dependence on $\|\theta_\ast\|$. 





% By contrast, the regret of \texttt{OFULog} from \cite{abeille2021instance} is $O(d\sqrt{T\dmu(x_\ast^\T\theta_\ast)\|\theta_\ast\|^2} +  d^2\min(\kappa, K)\log(T))$. In particular, \HOMER improves upon the result of \texttt{OFULog} by at least factor of $\sqrt{d\|\theta_\ast\|^2}$ though it should be mentioned that Corollary~\ref{cor:minimax_regret} is an upper bound to the result of Theorem~\ref{thm:mix_regret_complexity}. 

% \subsection{Sketch of Proofs}
% In this section we sketch the proofs of Lemma~\ref{lem:mean_param_bound} and corollary~\ref{cor:minimax_regret} to highlight the technical innovations of this work deferring precise details to the appendix. 

% \begin{proof}[Proof sketch of Lemma~\ref{lem:mean_param_bound}]

% Rewrite
% \begin{align*}
%     \mu(\htheta_t^\top x) - \mu(\theta_\ast^\top x) = \frac{\mu(\htheta_t^\top x) - \mu(\theta_\ast^\top x)}{x^\top (\htheta_t - \theta_\ast)} x^\top (\htheta_t - \theta_\ast) =: \alpha_x(\htheta_t, \theta_\ast)  \cdot x^\top (\htheta_t - \theta_\ast)
% \end{align*}
% Intuitively, $\alpha_x(\htheta_t, \theta_\ast)$ approximates $\dmu(\theta_\ast^\top x)$ and the above is akin to a first order Taylor expansion of $\mu(z)$ around $\theta_\ast^\top x$. Using self-concordance, e.g. \citep[Lemma 9]{faury2020improved} one can show that 
% \begin{align*}
%     \alpha_x(\htheta_t, \theta_\ast) \leq e\cdot \dmu(\theta_\ast^\top x)
% \end{align*}
% provided the warmup condition is satisfied. Then we use the natural parameter deviation bound given in \citet[Theorem 10]{jun2020improved} to control $|x^\top (\htheta_t - \theta_\ast)|$, completing the proof.
% \end{proof}

% Next, we sketch the proof of Corollary~\ref{cor:minimax_regret} which connects our regret bound to those of \citep[]{faury2020improved} and \citep[]{jun2020improved}.

% \begin{proof}[Proof sketch of Corollary \ref{cor:minimax_regret}]

% In the proof of Theorem~\ref{thm:mean_param_regret}, we show that the regret of \HOMER is 
% \begin{align*}
%     d\gamma(d) + \sum_k 2^k \min_\lambda \max_x
% \end{align*}

% \end{proof}


% Start with CI, then the regret bound, then finally just prove corollary 6?
% \textcolor{red}{Sketch of proofs}





==> algorithm.tex <==
\section{Elimination Based Algorithm}

\begin{algorithm}[ht] \caption{Elimination in mean parameter space}
    \label{alg:exp-design-regret}
    \begin{algorithmic}
        \Require{$\epsilon$, $\delta$, $\X$, $\kappa_0$, rounding procedure}
        \State{$k=1, \X_1 = \X$, $\gamma(d, \S, \delta) = d + \log(6(2+|\S|)/\delta)$}
        \State {$\hat\theta_0\leftarrow$ \textbf{BurnIn}($\X, \kappa_0$)}  \Comment{Burn-in phase}
        \While{$|\X_k| > 1$ } \Comment{Elimination phase}
        % \State  $\delta_k = \delta/(2|\X|k^2)$
        \State  $\delta_k = \delta/(4(2+|\X|)|\X|k^2)$
        % \State$f(\lambda) :=
        %         \gamma(d, |\X_k|, \delta_k)^{-1}\max_{x\in\X_k} \|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2$
        % \State $g(\lambda) :=2^{2k} 
        %         \max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda, \hat{\theta}_{0})^{-1}}^2$
        \State$f(\lambda) :=
                \max\left\{2^{2k} 
                \max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2, \gamma(d, |\X_k|, \delta_k)^{-1}\max_{x\in\X_k} \|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2\right\}$
        \State $\lambda_k = \arg\min_{\lambda\in \Delta_{\X_k}} f(\lambda)$
        \State{$n_k = \max\{3.5^2(1+\epsilon)\cdot e^3\cdot f(\lambda_k)\log(1/\delta_k), r(\epsilon)\}$}
        % \State $\lambda_k = \arg\min_{\lambda\in \Delta_{\X_k}} g(\lambda)$ \Comment{Note that this is a distribution over $\X_k$}
        \State{$x_1, \cdots x_{n_k}=\rdp(\lceil n_k\rceil, \lambda_k, \epsilon) $}
        % \State{$n_k^B =  \lceil f(\lambda_k^B)\lambda_k^B\rceil\in \Delta_{\X_k}$ and $n_k =  \lceil f(\lambda_k^B)\lambda_k\rceil\in \Delta_{\X_k}$}
        % \State{Pull each $x_i$, $n_{k,i}$ and $n_{k,i}^B$ times.} 
        \State{Observe rewards $y_1, \cdots, y_{n_k}$ and Compute the MLE $\hat\theta_k$ with $ \{(x_i,y_i)\}_{i=1}^{n_k}$. }
        % \State{$\hat{x}_k = \arg\max_{x\in\X_k} \hat\theta_k^\top x$}
        \State{$\X_{k+1}\leftarrow \X_k \setminus \left\{x\in \X_k:\max_{x'\in \X_k}\mu(x'^T\hat{\theta}_k) - \mu(x^T\hat{\theta}_k) \geq 2\cdot 2^{-k}\right\}$}
        \State{$k\gets k+1$}
		\EndWhile
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{BurnIn}
	\begin{algorithmic}
        \Require $\X, \kappa_0, \epsilon$
		\State $\lambda_0 = \arg\min_{\lambda\in \Delta_{\X}}\max_{x\in \mathcal{X}} \|x\|_{A(\lambda)^{-1}}^{2}$ 
% 		\State $n_0 = 3\kappa_0^{-1}\gamma^{-1}\log(|\X|/\delta)$
		\State{$n_0 =  3(1+\epsilon)d\gamma(d)\log(2(2 + |\X|)|\X|/\delta) $ \kj{are we missing $\kappa_0$ here?}}
		\State $x_1, \cdots, x_{n_0}\leftarrow \rdp(\lceil n_0\rceil, \lambda_0, \epsilon)$
        \State Pull each $x_i$, $n_{0,i}$ times and observe associated rewards $y_1, \cdots, y_{n_0}$.
		\State \Return MLE $\hat{\theta}_0$
	\end{algorithmic}
\end{algorithm}

% \begin{theorem}\label{thm:mean_param_regret}
% Define $\S_k = \{x\in \X:(x^{\ast}-x)^{\top}\theta^{\ast}\leq 2^{-k}\}$ and $\kappa = \max_{x\in \X_k} \dot\mu(x^{\top}\theta^{\ast})$ Algorithm~\ref{alg:exp-design-regret} obtains a regret 
% \begin{align*}
%     R \leq \sum_{k=1}^{\lceil \log_2(1/\Delta)\rceil} 2^{k}\min_{\lambda\in \Delta_{S_k}}\max_{x\in \X_k} \dot\mu(x^{\top}\theta^{\ast})^2\|x\|_{H(\theta^{\ast}, \lambda)^{-1}}^2\log(1/\delta) + (d^2 + \kappa^{-1})\lceil\log_2(1/\Delta)\rceil\log(1/\delta)
% \end{align*}
% In particular, we have an instance dependent bound,
% \[R_T\lesssim \frac{\min_{\lambda\in \Delta_{\X}}\max_{x\in \X} \dot\mu(x^{\top}\theta^{\ast})^2\|x\|_{H(\theta^{\ast}, \lambda)^{-1}}^2 \log(T)}{\Delta}\]
% and a minimax bound

% \end{theorem}
\begin{theorem}\label{thm:mean_param_regret}
Fix $\delta \leq e^{-1}$. Define $\S_k = \{x\in \X:\mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx)\leq 8\cdot 2^{-k}\}$ and $\kappa = \max_{x\in \X_k} \dot\mu(x^{\top}\theta^{\ast})$. 
Define $T' := T - \lceil3(1+\epsilon)d\gamma(d)\log(2(2 + |\X|)|\X|/\delta)\rceil$ and assume $T' > 0$. With probability at least $1-\delta$, 
algorithm~\ref{alg:exp-design-regret}, for any $\nu > 0$ obtains a regret 
\begin{align*}
    R & \leq \lceil3(1+\epsilon)d\gamma(d)\log(2(2 + |\X|)|\X|/\delta)\rceil + T'\nu + (4r(\epsilon) + 1)\lceil\log_2(8 (\Delta \vee \nu)^{-1})\rceil + \\
    & 8\cdot 3.5^2(1+\epsilon)\cdot e^3\cdot\log\left(\frac{4(2+|\X|)|X|\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil^2}{\delta}\right)\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}  \min_{\lambda}f(\lambda)
\end{align*}
where 
\begin{align*}
    f(\lambda) \leq 3e\max\left\{2^{2k} 
                \max_{x\in\S_k} \dot{\mu}(x^T\theta_\ast)\|x\|_{H(\lambda, \theta_\ast)^{-1}}, \gamma(d, |\S_k|, \delta_k)^{-1}\max_{x\in\S_k} \|x\|_{H(\lambda, \theta_\ast)^{-1}}^2\right\}.
\end{align*}
\end{theorem}
\textbf{To discuss:}
\begin{enumerate}
    \item How can we avoid per-round burn in? Taking $\theta_0$ at the beginning may not work because $\gamma(d)$ depends on $\delta$ and changes round to round
    \item If we have to burn in in each round, how can we mix the distributions? 
\end{enumerate}
\begin{lemma}[Lemma 4, \cite{jun2020improved}]\label{lem:burnin_guarantee}
For $\delta < e^{-1}$, with probability greater than $1-\delta$, for any $\lambda \in \Delta_{\X}$, $\frac{1}{3}H(\lambda, \theta_\ast) \preceq H(\lambda, \hat{\theta}_0) \preceq 3H(\lambda, \theta_\ast)$. Furthermore, $|\bx^T(\hat{\theta}_0 - \theta_\ast)| \leq 1$.  
\end{lemma}


\begin{lemma}\label{lem:mean_param_regret_correct}
For any $\delta \leq e^{-1}$, with probability at least $1-\delta$, for all rounds $k\in \N$ we have that $\bx_\ast \in \X_k$ and $\max_{\bx\in \X_k}\mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx) \leq 8\cdot 2^{-k}$. 
\end{lemma}

\begin{proof}
In each round $k$
\begin{align*}
    \max_{x\in\X_k} \|x\|_{H_{n_k}({\theta}_{\ast})^{-1}}^2 & \leq \frac{(1+\epsilon)}{n_k}\max_{x\in\X_k} \|x\|_{H(\lambda_k, {\theta}_{\ast})^{-1}}^2 \\
    & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} \frac{3(1+\epsilon)}{n_k}\max_{x\in\X_k} \|x\|_{H(\lambda_k, \hat{\theta}_{0})^{-1}}^2\\
    & \leq \gamma(d, |\X_k|, \delta_k)^{-1}
\end{align*}
where the final step follows from the definition of $n_k^B$. Then, by Corollary~\ref{cor:mean_param_bound}, and Lemma~\ref{lem:burnin_guarantee},
we have that with probability $1-\delta_k$, 
\begin{align*}
    |\mu(\hat{\theta}_k^T\bx_s) - \mu({\theta}_\ast^T\bx_s)| &\leq 3.5e\sqrt{\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H_{n_k}(\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}\\
    & \leq 3.5e\sqrt{\frac{(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k,\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k}}\\
    & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} 3.5e\sqrt{\frac{3(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k,\theta_k)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k}}\\
    & \stackrel{\text{Lemma 5, \cite{jun2020improved}}}{\leq} 3.5e\sqrt{\frac{3e(1+\epsilon)\dot{\mu}(\bx^T\hat{\theta}_k)^2\|\bx\|_{H(\lambda_k,\theta_k)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k}}\\
    & \leq 2^{-k}
\end{align*}
for all $\bx \in \X_k$. Via a union bound over the rounds, this condition holds in every round. 
First, we show that the best arm, $\bx_\ast$ is never eliminated. We have that $\X_1 = \X$. Assume the inductive hypothesis that $\bx_\ast \in \X_k$. For any $\bx \in \in \X_k$,
\begin{align*}
    \mu(\htheta_k^T\bx) - \mu(\htheta_k^T\bx_\ast) 
    & = \mu(\htheta_k^T\bx) - \mu(\theta_\ast^T\bx) + \mu(\theta_\ast^T\bx) - \mu(\theta_\ast^T\bx_\ast) + \mu(\theta_\ast^T\bx_\ast) -\mu(\htheta_k^T\bx_\ast) \\
    & \leq \mu(\htheta_k^T\bx) - \mu(\theta_\ast^T\bx) + \mu(\theta_\ast^T\bx_\ast) -\mu(\htheta_k^T\bx_\ast) \\
    & \leq 2\cdot 2^{-k}.
\end{align*}
Hence, $\bx_\ast \in \X_{k+1}$. Next, we show that for any $\bx$ such that $\mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx) > 4\cdot 2^{-k}$, $\bx \not\in \X_{k+1}$. 
\begin{align*}
    \mu(\htheta_k^T\bx_\ast) - \mu(\htheta_\ast^T\bx)
    & = \mu(\htheta_k^T\bx_\ast)- \mu(\theta_\ast^T\bx_\ast) + \mu(\theta_\ast^T\bx_\ast) -  \mu(\theta_\ast^T\bx) + \mu(\theta_\ast^T\bx)  -\mu(\htheta_\ast^T\bx) \\
    & > 2\cdot 2^{-k}
\end{align*}
which implies that $\bx \not\in \X_{k+1}$. Taken together, these statements implies that the regret of any arm present in round $k$ is at most $8\cdot 2^{-k}$. 
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:mean_param_regret}]
% \begin{enumerate}
%     \item Use Caratheodory's theorem to show the support of all designs is bounded by $d(d+1)/2$
%     \item Show that the confidence width holding leads to filtering on gaps
%     \item show that the number of samples in the burn in is bounded by $\kappa^{-1}$
%     \item can we switch between $\theta_0$ and $\theta_\ast$ for $\dot{\mu}$ space?
% \end{enumerate}
Let $T' := T - \lceil3(1+\epsilon)d\gamma(d)\log(2(2 + |\X|)|\X|/\delta)\rceil$ be the number of samples taken after the burn in procedure. We assume $T' > 0$. Since all rewards are bounded by $1$, the burn in contributes at most $\lceil3(1+\epsilon)d\gamma(d)\log(2(2 + |\X|)|\X|/\delta)\rceil$ to the total regret. We proceed by bounding the remaining $T'$ samples following burn in. Let $n_k^i$ denote the number of times $\bx_i$ is pulled in round $k$ and let $\lambda_k^i$ denote the fraction of the allocation placed on arm $i$. 
\begin{align*}
    R_{T'} & = \sum_{x \in \X \backslash \{x^\ast\}} \Delta_x T_x \\
    %%%%%%%%%%%%%%
    & \leq T'\nu + \sum_{k=1}^\infty \sum_{x \in \X \backslash \{x^\ast\}: \Delta_x > \nu} \Delta_x n_k^i \\
    %%%%%%%%%%%%%%
    & \leq T'\nu + \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} \sum_{x \in \X \backslash \{x^\ast\}: \Delta_x > \nu} \Delta_x n_k\lambda_k^i \\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu + 8\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} \lceil n_k\rceil \\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu + 1 + \log_2(8 (\Delta \vee \nu)^{-1}) + 8\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} n_k \\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu + \lceil\log_2(8 (\Delta \vee \nu)^{-1})\rceil + 8\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} n_k \\
    %%%%%%%%%%%%%%%%%%
    & = T'\nu + \lceil\log_2(8 (\Delta \vee \nu)^{-1})\rceil + 8\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} \max\{3.5^2(1+\epsilon)\cdot e^3\cdot f(\lambda_k)\log(1/\delta_k), r(\epsilon)\}\\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu + (4r(\epsilon) + 1)\lceil\log_2(8 (\Delta \vee \nu)^{-1})\rceil + \\
    & 8\cdot 3.5^2(1+\epsilon)\cdot e^3\cdot\log\left(\frac{4(2+|\X|)|X|\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil^2}{\delta}\right)\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}  f(\lambda_k)
\end{align*}
Finally, note that the term 
\begin{align*}
    & \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}  f(\lambda_k) \\
    & = \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} \min_\lambda \max\left\{2^{2k} 
                \max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2, \gamma(d, |\X_k|, \delta_k)^{-1}\max_{x\in\X_k} \|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2\right\}
\end{align*}
By Lemma~\ref{lem:mean_param_regret_correct}, we have that $\X_k \subset \{\bx \in \X: \mu(\theta_\ast^T\bx) - \mu(\theta_\ast^T\bx) \leq 8\cdot 2^{-k}\} =: \S_{k}$. Hence, we may upper bound maximization as being over $\S_k$ instead. Combinging this with Lemma 5  of \cite{jun2020improved}, this we have that 
\begin{align*}
    & \max\left\{2^{2k} 
                \max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2, \gamma(d, |\X_k|, \delta_k)^{-1}\max_{x\in\X_k} \|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2\right\}\\
    & \leq 3e\max\left\{2^{2k} 
                \max_{x\in\S_k} \dot{\mu}(x^T\theta_\ast)\|x\|_{H(\lambda, \theta_\ast)^{-1}}, \gamma(d, |\S_k|, \delta_k)^{-1}\max_{x\in\S_k} \|x\|_{H(\lambda, \theta_\ast)^{-1}}^2\right\}
    &
\end{align*}
Adding the contribution to the regret of the burn in completes the proof. 
% We proceed by analyzing each bracketed term separately. We begin with the regret due to burn in. 
% \begin{align*}
%     \sum_{k=1}^\infty \sum_{x \in \X \backslash \{x^\ast\}: \Delta_x > \nu} & \Delta_x \lceil \lambda_{k,x}^B \cdot f(\lambda_{k}^B)\rceil \\
%     & \lesssim \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}(|\text{support}(\lambda_{k}^B)| + \gamma^{-1} \min_{\lambda}\max_{x\in \X_k} \|x\|_{H(\lambda, \hat{\theta}_0)^{-1}}^2 \log(2k^2|\X|/\delta)) \\
%     & \lesssim \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}(|\text{support}(\lambda_{k}^B)| + \gamma^{-1} \min_{\lambda}\max_{x\in \X_k} \|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(2k^2|\X|/\delta)) \\
%     & \lesssim \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}(d^2 + \gamma^{-1} \kappa_0^{-1} \log(2k^2|\X|/\delta)) \\
%     & \lesssim (d^2 + \gamma^{-1} \kappa_0^{-1} \log(2\log_2^2(8 (\Delta \vee \nu)^{-1})|\X|/\delta))
% \end{align*}
% Next, we control the regret due to the design directly. 
% \begin{align*}
%     \sum_{k=1}^\infty & \sum_{x \in \X \backslash \{x^\ast\}: \Delta_x > \nu}  \Delta_x \lceil \lambda_{k,x} \cdot g(\lambda_{k})\rceil \\
%     & \lesssim \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}(|\text{support}(\lambda_{k})| +  2^{2k}\min_{\lambda}\max_{x\in \X_k} \dot{\mu}(x^T\hat{\theta}_0)^2\|x\|_{H(\lambda, \hat{\theta}_0)^{-1}}^2 \log(2k^2|\X|/\delta)) \\
%     & \lesssim \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}(|\text{support}(\lambda_{k})| +  2^{2k}\min_{\lambda}\max_{x\in \X_k} \dot{\mu}(x^T\theta_\ast)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(2k^2|\X|/\delta)) \\
%     & \lesssim \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}(d^2 +  2^{2k}\min_{\lambda}\max_{x\in \X_k} \dot{\mu}(x^T\theta_\ast)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(2k^2|\X|/\delta)) \\
%     & \leq d^2 \lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil + \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{k} \min_{\lambda}\max_{x\in \X_k} \dot{\mu}(x^T\theta_\ast)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(2k^2|\X|/\delta) \\
%     & \leq d^2 \lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil + \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{k} \min_{\lambda}\max_{x\in \S_k} \dot{\mu}(x^T\theta_\ast)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(2k^2|\X|/\delta)
% \end{align*}
% Putting all pieces together, we have that 
% \begin{align*}
%     R_T & \lesssim T\nu + d^2\log_2((\Delta \vee \nu)^{-1}) + \gamma^{-1} \kappa_0^{-1} \log(2\log_2^2(8 (\Delta \vee \nu)^{-1})|\X|/\delta) \\
%     & \hspace{1cm} + \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{k} \min_{\lambda}\max_{x\in \S_k} \dot{\mu}(x^T\theta_\ast)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(2k^2|\X|/\delta)
% \end{align*}
% Recall that there is an additional $\kappa^{-1}\lambda^{-1}\log(2|\X|/\delta)$ regret due to the initial burn in. Adding this and setting $\nu = 0$, we see that up to doubly logarithmic terms, 
% \begin{align*}
%     R_T \leq & \kappa^{-1}\gamma^{-1}\log(|\X|/\delta) (1 + \log_2(1/\Delta)) + d^2\log_2(1/\Delta) \\
%     & +  \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{k} \min_{\lambda}\max_{x\in \S_k} \dot{\mu}(x^T\theta_\ast)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(2k^2|\X|/\delta) \\
%     & \approx (d^2 + \kappa^{-1}\lambda^{-1}\log(|\X|/\delta)) \log_2(1/\Delta) +  \sum_{k=1}^{\lceil \log_2(1/\Delta)\rceil} 2^{k} \min_{\lambda}\max_{x\in \S_k} \dot{\mu}(x^T\theta_\ast)^2\|x\|_{H(\lambda, \theta_\ast)^{-1}}^2 \log(k^2|\X|/\delta)
% \end{align*}
\end{proof}












\section{Extensions}

\begin{itemize}
  \item Instead of assigning certain samples for satisfying the burnin condition, we could use a burnin sample just once and call it $\hat\theta_0$.
  Then, we can use the regularizer $\|\theta - \hat\theta_{0}\|^2$. Or, perhaps this is better: $ \|\theta - \hat\theta_{0}\|_{H(\hat\theta_{0})}^2$.
  \item Empirically show that our algorithm can work better than Faury's algorithm by leveraging the informative arm. Caveat: but the informative arm will be eliminated soon? hopefully not eliminated too fast.
  \item Change the design problem so we achieve asymptotic optimality up to a constant factor.
  \begin{itemize}
      \item How about achieving the minimax optimality at the same time? (This is interesting even for the standard linear bandits.)
      I imagine that we will design an algorithm so it initially behaves like the elimination algorithm above, but after some time point switch to the design problem for regret minimization that involves estimated gaps.
      I imagine that after some time point we will start reviving eliminated arms (call them zombie arms) and include them in the design problem because they could be the informative arms.
      Here, we should try to revive arms from small gaps to large gaps. 
  \end{itemize}
  \item Can we avoid paying $\kappa^{-1}$ in the burnin? 
  \item Recall that we have an online estimation version as well. Perhaps we can put it in the paper together?
\end{itemize}


==> conf_widths.tex <==
% \section{A bound for regret minimization}

% In this section, we quickly note how to alter the proof of confidence width on the natural parameter to control $\max_{s}|\bx_s(\hat{\theta} -\theta_\ast)|$. All notation is borrowed from the proof of the original confidence width. 

% \begin{theorem}\label{thm:natural_param_max}
% Fix $\delta \leq e^{-1}$. Let $\hat{\theta}_t$ denote the MLE estimate for a fixed design $\bx_1, \cdots, \bx_t$. Let $t_{\text{eff}}$ denote the number of distinct vectors in $\{\bx_s\}_{s=1}^t$. For any $c \in (0,1)$, if $\max_s\|\bx_s\|_{H^{-1}} =: \xi_t \leq \frac{\sqrt{1+c} - 1}{\sqrt{\log(2t_{\text{eff}}/\delta)}}$, then 
% \begin{align}
%     \max_{s}|\bx_s^T(\hat{\theta} - \theta^\ast)| \leq \frac{1}{1-c}\left(2\xi_t\sqrt{\log(2t_{\text{eff}}/\delta)} + \xi_t^2\log(2t_{\text{eff}}/\delta) \right)
% \end{align}
% with probability at least $1-\delta$. In particular, under the burnin condition,
% \[\max_{s}|\bx_s^T(\hat{\theta} - \theta^\ast)| \leq \frac{c}{1-c}\]
% \end{theorem}

% \begin{proof}
% First, we have that
% \begin{align}\label{eq:two_term_decomp}
%     |\bx^T(\theta_t - \theta_\ast)| = |\bx^TG^{-1}z_t| \leq |\bx^TH^{-1}z_t| + |\bx^TH^{-1}EG^{-1}z_t|.
% \end{align}

% We begin by analyzing the second sum.
% To avoid using Cauchy-Schwarz which will de-couple $\bx_s$ from the deviation of $\hat{\theta}_t - \theta_\ast$, we first require a result on the trace of a product. 
% \begin{lemma}[Von Neumann, \cite{von1937some}]
% Let $A, B\in \R^{n\times n}$ be matrices with singular values $a_1 \geq a_2 \geq \cdots \geq a_n$ and $b_1 \geq b_2 \geq \cdots \geq b_n$. Then $\text{Trace}(AB) \leq \sum_{i=1}^n a_i b_i$. 
% \end{lemma}
% Applying this, we see that
% \begin{align*}
%     |\bx^TH^{-1}EG^{-1}z_t| = |\text{Trace}(\bx^TH^{-1}EG^{-1}z_t)|
%     &= |\text{Trace}(z_t\bx^TH^{-1}EG^{-1})|\\
%     &\leq \|z_t\bx^TH^{-1}\|\cdot \|EG^{-1}\| \tag{Rank$(z_t\bx^TH^{-1})=1$}\\
%     &= |\bx^TH^{-1}z_t|\cdot \|EG^{-1}\|\\
%     &= |\bx^TH^{-1}z_t|\cdot \|I - HG^{-1}\| \tag{$ E = G -H$}.
% \end{align*}
% Hence, we may bound Equation~\eqref{eq:two_term_decomp}
% $$|\bx^T(\hat{\theta}_t - \theta_\ast)| \leq (1 +  \|I - HG^{-1}\|) |\bx^TH^{-1}z_t|. $$
% Observe that 
% \begin{align*}
%     \|I - HG^{-1}\| & = \max_{x: \|x\|=1} \max\left\{x^T(I - HG^{-1})x, \ x^T(HG^{-1}-I)x\right\} \\
% & = \max_{x: \|x\|=1} \max\left\{1 - x^THG^{-1}x, \ x^THG^{-1}x - 1\right\} \\
% & = \max\left\{1 - \min_{x: \|x\|=1}x^THG^{-1}x, \ \max_{x: \|x\|=1} x^THG^{-1}x - 1\right\}
% \end{align*}
% By the proof of Lemma 2 in the original bound, we have that
% $$G \succeq \frac{1}{1+D}H $$
% for $D = \max_{s \in [t]}|\bx_s^T(\hat{\theta}_t - \theta_\ast)|$. 
% Following its proof, by Lemma 9 of \cite{faury2020improved}, we have that 
% $$ \alpha_s(\hat{\theta}, \theta_\ast) \leq \max_s \frac{e^{|\bx_s(\hat{\theta}_t - \theta_\ast)| }-1}{|\bx_s(\hat{\theta}_t - \theta_\ast)|} \ \dot{\mu}(\bx_s^T\theta_2) \leq e^{|\bx_s(\hat{\theta}_t - \theta_\ast)|} \ \dot{\mu}(\bx_s^T\theta_2) $$
% Applying this, 
% \begin{align*}
%     G = \sum_{s=1}^t\alpha_s(\hat{\theta}_t, \theta_\ast)\bx_s\bx_s^T \preceq \max_{s\in [t]}e^{|\bx_s^T(\hat{\theta}_t - \theta_\ast)|}\sum_{s=1}^T\dot{\mu}(\theta_\ast^T\bx_s)\bx_s\bx_s^T = e^D H.
% \end{align*}
% Taken together, we have 
% \begin{align*}
%     \frac{1}{1+D}H \preceq G \preceq e^D H,
% \end{align*}
% which implies 
% \begin{align*}
%     e^{-D}I \preceq HG^{-1} \preceq (1 + D) I
% \end{align*}
% and 
% \begin{align*}
%     e^{-D} \leq \bx^T HG^{-1} \bx  \leq (1 + D) \ \forall \bx: \|\bx\|=1.
% \end{align*}
% Plugging this in to control $\|I - HG^{-1}\|$, we have that 
% \begin{align*}
%     \|I - HG^{-1}\|\leq \max\{1 - e^{-D}, D\} \leq D. 
% \end{align*}
% Therefore, 
% \begin{align*}
%     |\bx^T(\hat{\theta}_t - \theta_\ast)| \leq (1 +  D) |\bx^TH^{-1}z_t|.
% \end{align*}
% To control $|\bx^TH^{-1}z_t|$, we can modify Lemma 1 in the original proof slightly. 
% We have using lemma 1 for a generic $\bx$ that with probability $1-\delta$
% \begin{align*}
%     \bx^TH^{-1}z_t \leq \phi\|\bx\|_{H^{-1}}^2 + \frac{1}{\phi}\log(1/\delta)
% \end{align*}
% for $\phi$ satisfying
% $|\phi| \leq \frac{1}{\max_{s}|\langle\bx, H^{-1}\bx_s\rangle|}$.
% Define $\xi_t = \max_s \|\bx_s\|_{H^{-1}}$. In the specific case that we wish to control $\bx_s^TH^{-1}z_t$ 
% for $s \in [t]$ (i.e., $\bx\in \{\bx_1, \cdots \bx_t\}$),
% choose 
% $$\phi = \min \left(\sqrt{\frac{\log(1/\delta)}{\|\bx_s\|_{H^{-1}}^2}}, \frac{1}{\max_{r\in [t]}|\langle\bx_s, H^{-1}\bx_r\rangle|}\right).$$
% Plugging this in and union bounding over the identical argument for $-\bx_s^TH^{-1}
% z_t$, we have that
% % \begin{align*}
% %   |\bx_s^TH^{-1}z_t| \leq \min\left(2\|\bx_s\|_{H^{-1}}\sqrt{\log(2/\delta)}, \frac{\|\bx_s\|_{H^{-1}}^2}{B} + B\log(2/\delta) \right)
% % \end{align*}
% \begin{align*}
%   |\bx_s^TH^{-1}z_t| & \leq 2\|\bx_s\|_{H^{-1}}\sqrt{\log(2/\delta)} + \max_{r\in [t]}|\langle\bx_s, H^{-1}\bx_r\rangle|\log(2/\delta)\\
%   & \leq 2\|\bx_s\|_{H^{-1}}\sqrt{\log(2/\delta)} + \|\bx_s\|_{H^{-1}}\xi_t\log(2/\delta)
% \end{align*}
% which implies
% \begin{align*}
%     |\bx_s^T(\hat{\theta}_t - \theta_\ast)| \leq (1+D) \left(2\|\bx_s\|_{H^{-1}}\sqrt{\log(2/\delta)} + \|\bx_s\|_{H^{-1}}\xi_t\log(2/\delta) \right).
% \end{align*}
% Next, let $t_{\text{eff}}$ denote the number of unique vectors in the design $\{\bx_1, \cdots, \bx_t\}$. Via a union bound, the above hold for all $\bx_s$ and hence, the max. Therefore, 
% % \begin{align*}
% %     \max_s|\bx_s^T(\hat{\theta}_t - \theta_\ast)| = D \leq (1 + D)\max_s\min\left(2\|\bx_s\|_{H^{-1}}\sqrt{\log(2t_{\text{eff}}/\delta)}, \frac{\|\bx_s\|_{H^{-1}}^2}{B} + B\log(2t_{\text{eff}}/\delta) \right).
% % \end{align*}
% \begin{align*}
%     \max_s|\bx_s^T(\hat{\theta}_t - \theta_\ast)| = D &\leq (1 + D)\max_s\left(2\|\bx_s\|_{H^{-1}}\sqrt{\log(2t_{\text{eff}}/\delta)} + \|\bx_s\|_{H^{-1}}\xi_t\log(2t_{\text{eff}}/\delta) \right)\\
%     & = (1 + D)\left(2\xi_t\sqrt{\log(2t_{\text{eff}}/\delta)} + \xi_t^2\log(2t_{\text{eff}}/\delta) \right).
% \end{align*}
% Next, note that for $\psi := 2\xi_t\sqrt{\log(2t_{\text{eff}}/\delta)} + \xi_t^2\log(2t_{\text{eff}}/\delta)$ and any $c \in (0, 1)$, we have that $\psi \leq c$ implies
% \begin{align*}
%     D \leq \frac{\psi}{1 - \psi} \leq \frac{1}{1-c}\psi.
% \end{align*}
% $\psi \leq c$ is implied by 
% \begin{align*}
%     \xi_t \leq \frac{\sqrt{1+c} - 1}{\sqrt{\log(2t_{\text{eff}}/\delta)}}. 
% \end{align*}
% Putting this together, we have that
% \begin{align*}
%     \max_{s}|\bx_s^T(\hat{\theta} - \theta^\ast)| \leq \frac{1}{1-c}\left(2\xi_t\sqrt{\log(2t_{\text{eff}}/\delta)} + \xi_t^2\log(2t_{\text{eff}}/\delta) \right)
% \end{align*}
% for any $c \in (0,1)$ as long as $\max_s\|\bx_s\|_{H^{-1}} =\xi_t \leq \frac{\sqrt{1+c} - 1}{\sqrt{\log(2t_{\text{eff}}/\delta)}}$.  
% \end{proof}

\section{Bounds in mean parameter space}

In this section, we provide a confidence width for controlling the deviation of the mean parameter instead of the natural parameter.

% \begin{theorem}
% Fix $\delta \leq e^{-1}$. Let $\hat{\theta}_t$ denote the MLE estimate for a fixed design $\bx_1, \cdots, \bx_t$. Let $t_{\text{eff}}$ denote the number of distinct vectors in $\{\bx_s\}_{s=1}^t$. For any $c \in (0,1)$, if $\max_s\|\bx_s\|_{H^{-1}} =: \xi_t \leq \frac{\sqrt{1+c} - 1}{\sqrt{\log(2t_{\text{eff}}/\delta)}}$, then 
% \begin{align}
%     \max_{s\in [t]}|\mu(\bx_s^T\hat{\theta}_t) - \mu(\bx_s^T{\theta}_\ast)| \leq e^{\frac{c}{1-c}}\frac{1 + \sqrt{1+c}}{1-c}\max_{s\in [t]}\dot{\mu}(\bx_s^T\theta_\ast)\|\bx_s\|_{H^{-1}}\sqrt{\log(2t_\text{eff}/\delta)}
% \end{align}
% with probability at least $1-\delta$.
% \end{theorem}
\begin{corollary}\label{cor:mean_param_bound}
Fix $\delta \leq e^{-1}$. Let $\hat{\theta}_t$ denote the MLE estimate for a fixed design $\{\bx_1, \cdots, \bx_t\} \subset \X$. Let $t_{\text{eff}}$ denote the number of distinct vectors in $\{\bx_s\}_{s=1}^t$. Let $\gamma(d) = d + \log(6(2+ t_\text{eff})/\delta)$. Assume that $\xi_t^2 := \max_{\bx\in \X}\|\bx\|_{H_t(\theta_\ast)^{-1}}^2 \leq \gamma(d)^{-1}$.
Then with probability $1-\delta$, 
\begin{align}
    |\mu(\bx^T\hat{\theta}_t) - \mu(\bx^T{\theta}_\ast)| \leq 350\dot{\mu}(\bx^T\theta_\ast)\|\bx\|_{H_t(\theta_\ast)^{-1}}\sqrt{\log(2(2 + t_\text{eff})|\X|/\delta)}. 
\end{align}
for each $\bx \in \X$. Furthermore, if $|\bx^T(\hat{\theta}_t - \theta_\ast)| \leq D$, then the leading constant is $3.5\cdot e^D$. 
\end{corollary}
\begin{remark}
The constant of $350$ is largely a product of the burn in condition. If instead the burn in condition was changed to $\xi_t^2 := \max_{\bx\in \X}\|\bx\|_{H_t(\theta_\ast)^{-1}}^2 \leq c\gamma(d)^{-1}$ for some $c > 0$, the constant would be $3.5 \cdot e^{c\cdot 3.5}$. For instance, $c = 1/3.5$ leads to a constant of $10$.
\end{remark}

\begin{proof}
Given a fixed design $\{\bx_1, \cdots, \bx_t\}$, the condition that $\max_{\bx_s \in \{\bx_1, \cdots, \bx_t\}}\|\bx_s\|_{H_t(\theta_\ast)^{-1}}^2 \leq \max_{\bx\in \X}\|\bx\|_{H_t(\theta_\ast)^{-1}}^2 \leq \gamma(d)^{-1}$ implies that with probability at least $1-\delta$,
\begin{align*}
    |\bx_s^T(\hat{\theta}_t - \theta_\ast)| \leq 3.5 \|\bx_s\|_{H_t(\theta_\ast)^{-1}} \sqrt{\log(2(2+t_{\text{eff}})|\X|/\delta)}
\end{align*}
for each $\bx_s \in \X$ by Theorem 1 of \cite{jun2020improved}. 
We have that 
$$|\mu(\bx_s^T\hat{\theta}_t) - \mu(\bx_s^T{\theta}_\ast)| =  |\alpha_s(\hat{\theta}_t, \theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))|. $$
Using self concordance, we have that 
\begin{align*}
    |\alpha_s(\hat{\theta}_t, \theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))| 
    &\leq  \left|e^{\max_{s'}|\bx_{s'}^T(\hat{\theta}_t - {\theta}_\ast))|}\dot{\mu}(\bx_s^T\theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))\right|\\
    & \stackrel{\cE_1}{\leq} e^{D} \left|\dot{\mu}(\bx_s^T\theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))\right|.
\end{align*}
where $D := \max_{s'\in \X}|\bx_{s'}^T(\hat{\theta}_t - {\theta}_\ast))|$. Combining the above computation with the bound for each $\bx_s^T(\hat{\theta}_t - \theta_\ast)$ and taking a max over the possible $\bx's$, we have that
\begin{align*}
    |\mu(\bx_s^T\hat{\theta}_t) - \mu(\bx_s^T\theta_\ast)| \leq 3.5e^D \dot{\mu}(\bx_s^T\theta_\ast) \|\bx_s\|_{H_t(\theta_\ast)^{-1}} \sqrt{\log(2(2+t_{\text{eff}})|\X|/\delta)}
\end{align*}
Finally, note that on the condition that $\max_{\bx\in \X}\|\bx\|_{H_t(\theta_\ast)^{-1}}^2 \leq \gamma(d)^{-1}$,
\begin{align*}
    \max_s|\bx_s^T(\hat{\theta}_t - \theta_\ast)| & \leq \max_s 3.5 \|\bx_s\|_{H_t(\theta_\ast)^{-1}} \sqrt{\log(2(2+t_{\text{eff}})|\X|/\delta)} \\
    & \leq 3.5 \gamma(d)^{-1} \sqrt{\log(2(2+t_{\text{eff}})|\X|/\delta)} \\
    & \leq 3.5.
\end{align*}
Plugging in $D = 3.5$ and noting that $3.5 \cdot e^{3.5} \leq 350$ completes the proof. 
% Assume that the event from the proof of Theorem 1 of \cite{jun2020improved} that holds with probability at least $1-\delta$

% Assume event $\cE_1$ that holds with probability $1-\delta$ that
% \begin{align*}
%   |\bx_s^TH^{-1}z_t|  
%     \leq 2\|\bx_s\|_{H^{-1}}\sqrt{\log(2t_\text{eff}/\delta)} + \|\bx_s\|_{H^{-1}}\xi_t\log(2t_\text{eff}/\delta)
% \end{align*}
% for all $s\in [t]$. On $\cE_1$ and the condition that $\xi_t \leq \frac{\sqrt{1+c} - 1}{\sqrt{\log(2t_{\text{eff}}/\delta)}}$ for a fixed $c \in (0,1)$, the proof of Theorem~\ref{thm:natural_param_max} implies that
% \begin{align*}
%     \max_{s}|\bx_s^T(\hat{\theta} - \theta^\ast)| \leq \frac{1}{1-c}\left(2\xi_t\sqrt{\log(2t_{\text{eff}}/\delta)} + \xi_t^2\log(2t_{\text{eff}}/\delta) \right) =: \psi_t.
% \end{align*}
% We have that 
% $$\max_{s\in [t]}|\mu(\bx_s^T\hat{\theta}_t) - \mu(\bx_s^T{\theta}_\ast)| = \max_s |\alpha_s(\hat{\theta}_t, \theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))|. $$
% Using self concordance and the fact that $\alpha_s(\hat{\theta}_t, \theta_\ast) \geq 0$, 
% \begin{align*}
%     \max_s |\alpha_s(\hat{\theta}_t, \theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))| 
%     &\leq \max_s \left|e^{\max_{s'}|\bx_{s'}^T(\hat{\theta}_t - {\theta}_\ast))|}\dot{\mu}(\bx_s^T\theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))\right|\\
%     & \stackrel{\cE_1}{\leq} e^{\psi_t}\max_s \left|\dot{\mu}(\bx_s^T\theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))\right|.
% \end{align*}
% We now turn our attention to controlling the later maximum following similar ideas as the proof of Theorem~\ref{thm:natural_param_max}. 
% \begin{align*}
%     \left|\dot{\mu}(\bx_s^T\theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))\right| & = \left|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TG^{-1}z_t\right|\\
%     & \leq \left|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TH^{-1}z_t\right| + \left|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TH^{-1}EG^{-1}z_t\right|\\
%     & \leq (1 + \|I - HG^{-1}\|) \left|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TH^{-1}z_t\right|\\
%     & \leq (1 + \max_{s'}|\bx_{s'}^T(\hat{\theta}_t - {\theta}_\ast))|) \left|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TH^{-1}z_t\right|\\
%     & \stackrel{\cE_1}{\leq} (1 + \psi_t) \left|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TH^{-1}z_t\right|
% \end{align*}
% To control $|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TH^{-1}z_t|$, on event $\cE_1$ we have that for all $s \in [t]$
% \begin{align*}
%     |\dot{\mu}(\bx_s^T\theta_\ast)\bx^TH^{-1}z_t| \leq 2\dot{\mu}(\bx_s^T\theta_\ast)\|\bx_s\|_{H^{-1}}\sqrt{\log(2t_\text{eff}/\delta)} + \dot{\mu}(\bx_s^T\theta_\ast)\|\bx_s\|_{H^{-1}}\xi_t\log(2t_\text{eff}/\delta).
% \end{align*}
% Recall that on $\cE_1$ by the burn in condition, we have that $\xi_t \leq \frac{\sqrt{1+c} - 1}{\sqrt{\log(2t_{\text{eff}}/\delta)}}$ for a fixed $c \in (0,1)$. Therefore, we may plug this bound in to show that 
% \begin{align*}
%     |\dot{\mu}(\bx_s^T\theta_\ast)\bx^TH^{-1}z_t| \leq (1 + \sqrt{1+c})\dot{\mu}(\bx_s^T\theta_\ast)\|\bx_s\|_{H^{-1}}\sqrt{\log(2t_\text{eff}/\delta)}.
% \end{align*}
% Next, we may plug  this bound on the value of $\xi_t$ into the definition of $\psi_t$ to show that
% \begin{align*}
%     \psi_t =  \frac{1}{1-c}\left(2\xi_t\sqrt{\log(2t_{\text{eff}}/\delta)} + \xi_t^2\log(2t_{\text{eff}}/\delta) \right) \leq \frac{c}{1-c}. 
% \end{align*}
% Taken together, we have that 
% \begin{align*}
%     \max_{s\in [t]}|\mu(\bx_s^T\hat{\theta}_t) - \mu(\bx_s^T{\theta}_\ast)| & \stackrel{\cE_1}{\leq} (1 + \psi_t)e^{\psi_t}\max_s \left|\dot{\mu}(\bx_s^T\theta_\ast)(\bx_s^T(\hat{\theta}_t - {\theta}_\ast))\right| \\
%     & = (1 + \psi_t)e^{\psi_t}\max_{s\in [t]}\left|\dot{\mu}(\bx_s^T\theta_\ast)\bx_s^TG^{-1}z_t\right| \\
%     & \leq e^{\frac{c}{1-c}}\frac{1 + \sqrt{1+c}}{1-c}\max_{s\in [t]}\dot{\mu}(\bx_s^T\theta_\ast)\|\bx_s\|_{H^{-1}}\sqrt{\log(2t_\text{eff}/\delta)}.
% \end{align*}
\end{proof}

==> defs-kjun-v4-shared.tex <==

%_ better math font
\usepackage{amsthm,amsmath,bbm,amsfonts,amssymb}
\usepackage{dsfont} % require for using \mathds{1}
\usepackage{mathtools}
\usepackage{commath}
\mathtoolsset{showonlyrefs=false}

\usepackage{xspace}
% \usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[usenames,dvipsnames]{xcolor} % for color names


\usepackage{url}
\usepackage{cleveref} % must be loaded after amsthm

% \usepackage{wrapfig}
\usepackage[export]{adjustbox}
\def\imagetop#1{\vtop{\null\hbox{#1}}} % adjusting location of box in table
%- synctex
\synctex=1
% \pdfoutput=1  % for arxiv submission

% For algorithms
\usepackage{algorithm}
% \usepackage{algorithmic}

\usepackage{graphicx,tabularx}
\usepackage{multirow,hhline}% http://ctan.org/pkg/multirow
\usepackage{booktabs}% to use \midrule for drawing a horizontal line in align environment

\usepackage{capt-of}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

%\usepackage{enumitem}

\allowdisplaybreaks % This allows breaking multi-line equations

\usepackage{pbox} % new line in a table cell -- http://tex.stackexchange.com/questions/2441/how-to-add-a-forced-line-break-inside-a-table-cell

% for vertical alignment of includegraphics
%- http://tex.stackexchange.com/questions/101858/make-two-figures-aligned-at-top
\usepackage[export]{adjustbox}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\cm}{\ding{51}}%
\newcommand{\gyes}{{\color[rgb]{0,.8,0}\cmark}}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\xm}{\ding{55}}%
\newcommand{\rno}{{\color[rgb]{.8,0,0}\xmark}}

% define your comment color here
\newcommand{\jerry}[1]{{ \color[cmyk]{0,0.61,0.87,0}jerry: #1 }}
\newcommand{\rob}[1]{{ \color[rgb]{0,0.718,0.179}rob: #1 }}
\newcommand{\kwang}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}
\newcommand{\kw}[1]{{ \color[rgb]{1,0.279,0.998} #1 }}
%\newcommand{\kj}[1]{{\color{RedOrange}#1}}
\newcommand{\gray}[1]{{ \color[rgb]{.6,.6,.6} #1 }}
% \newcommand{\blue}[1]{{\color[rgb]{.3,.5,1}#1}}
\newcommand{\grn}[1]{{\color{ForestGreen}#1}}
\newcommand{\org}[1]{{\color{Orange}#1}}
\newcommand{\vio}[1]{{\color{Violet}#1}}
\newcommand{\red}[1]{{\color[rgb]{1,.1,.1}#1}}
\newcommand{\gr}[1]{{\color[rgb]{.8,.8,.8}#1}}

% %---------- setup theorem environment
% \usepackage{framed}
% \usepackage[most]{tcolorbox}
% \definecolor{kjgray}{rgb}{.7,.7,.7}

% \newtheoremstyle{kjstyle}
% {1ex} % Space above
% {\topsep} % Space below
% {\itshape} % Body font
% {} % Indent amount
% {\bfseries} % Theorem head font
% {.} % Punctuation after theorem head
% {.5em} % Space after theorem head
% {} % Theorem head spec (can be left empty, meaning `normal')

% \newtheoremstyle{kjstylenoitalic}
% {1ex} % Space above
% {\topsep} % Space below
% {} % Body font
% {} % Indent amount
% {\bfseries} % Theorem head font
% {.} % Punctuation after theorem head
% {.5em} % Space after theorem head
% {} % Theorem head spec (can be left empty, meaning `normal')

% \tcbset{kjboxstyle/.style={title={},breakable,colback=white,enhanced jigsaw,boxrule=1.3pt,sharp corners,colframe=kjgray,boxsep=0pt,coltitle={black},attach title to upper={},left=.8ex,bottom=.4em}}    
% %    ,title after break={Lemma \thelemma\ (continued)}}
% %}

%---------------- disabled for the moment.
%\newtheorem{theorem}{Theorem}
%
%
%\theoremstyle{kjstyle}\newtheorem{thm}{Theorem}
%\AtBeginEnvironment{thm}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{thm}{\end{tcolorbox}}%
%\theoremstyle{kjstyle}\newtheorem{lem}[thm]{Lemma}
%\AtBeginEnvironment{lem}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{lem}{\end{tcolorbox}}%
%%\theoremstyle{kjstyle}\newtheorem{lem}[thm]{Lemma}
%%\AtBeginEnvironment{lem}{\begin{tcolorbox}[kjboxstyle]}%
%%  \AtEndEnvironment{lem}{\end{tcolorbox}}%
%\theoremstyle{kjstyle}\newtheorem{prop}[thm]{Proposition}
%\AtBeginEnvironment{prop}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{prop}{\end{tcolorbox}}%
%\theoremstyle{kjstyle}\newtheorem{cor}[thm]{Corollary}
%\AtBeginEnvironment{cor}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{cor}{\end{tcolorbox}}%
%
%\theoremstyle{kjstyle}\newtheorem{defn}{Definition}
%\AtBeginEnvironment{defn}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{defn}{\end{tcolorbox}}%
%
%\theoremstyle{kjstyle}\newtheorem{ass}{Assumption}
%\AtBeginEnvironment{ass}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{ass}{\end{tcolorbox}}%
%\renewcommand\theass{A\arabic{ass}}
%
%
%\theoremstyle{kjstyle}\newtheorem{question}{Question}
%\AtBeginEnvironment{question}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{question}{\end{tcolorbox}}%
%% \renewcommand\theass{A\arabic{ass}}
%
%\theoremstyle{kjstylenoitalic}\newtheorem{remark}{Remark}
%\AtBeginEnvironment{remark}{\begin{tcolorbox}[kjboxstyle]}%
%  \AtEndEnvironment{remark}{\end{tcolorbox}}%


% %--------------- other ways to create box
% \newcommand{\kjunboxold}[1]{\vspace{.5em}\\\fbox{%
%     \begin{minipage}{\linewidth}
%       \centering #1
%     \end{minipage}%
%   }\vspace{.5em}}
% \def\lamp{\ensuremath{\lambda_\perp}}
% \usepackage{mdframed}
% \usepackage{lipsum}
% \definecolor{kjgray}{rgb}{.7,.7,.7}
% \makeatletter
% \newcommand{\kjunbox}[1]{\vspace{.4ex}
%   \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt]
%     #1
%   \end{mdframed}%
% }
% \makeatletter
% \newcommand{\kjunboxcenter}[1]{\vspace{.4ex}
%   \begin{mdframed}[linecolor=kjgray,innertopmargin=1.3ex,innerleftmargin=.4em,innerrightmargin=.4em,linewidth=1.3pt,userdefinedwidth=.8\linewidth,align=center]
%     %[linecolor=black,innerleftmargin=.4em,innerrightmargin=.4em,userdefinedwidth=.8\linewidth,align=center]
%     #1
%   \end{mdframed}%
% }
% \makeatother


% %--- to remove the space before paragraph : change 3.25ex to ...
% \makeatletter
% \renewcommand{\paragraph}{%
%   \@startsection{paragraph}{4}%
%   {\z@}{0.50ex \@plus 1ex \@minus .2ex}{-1em}%
%   {\normalfont\normalsize\bfseries}%
% }
% \makeatother

% %- https://tex.stackexchange.com/questions/72692/highlight-an-equation-within-an-align-environment-with-color-option
% %------- this makes a border that covers other part of the equation....
% \usepackage[customcolors,shade]{hf-tikz} % after {}, (right, below) and then (left, above) offset... I don't know how it works; done by trial-and-error.
% \newcommand{\hll}[2]{\tikzmarkin[set fill color=yellow!30]{#1}(0.02,-.08)(-0.02,0.3)#2\tikzmarkend{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
% \def\ddef#1{\expandafter\def\csname #1#1\endcsname{\ensuremath{\mathbb{#1}}}}
% \ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{{\boldsymbol{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSUVWXYZabcdeghijklmnopqrtsuvwxyz\ddefloop
%\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{\mathbf{#1}}}}
%\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname h#1\endcsname{\ensuremath{\hat{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrsuvwxyz\ddefloop % except for 't' because it is used by others
\def\ddef#1{\expandafter\def\csname hc#1\endcsname{\ensuremath{\widehat{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname t#1\endcsname{\ensuremath{\widetilde{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname r#1\endcsname{\ensuremath{\mathring{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrtsuvwxyz\ddefloop
\def\ddef#1{\expandafter\def\csname tc#1\endcsname{\ensuremath{\widetilde{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop


\def\hmu{{\ensuremath{\hat{\mu}}} }
\def\bhmu{{\ensuremath{\boldsymbol{\hat{\mu}}} }}

\def\SS{{\mathbb{S}}}

\DeclareMathOperator*{\argmax}{arg~max}
\DeclareMathOperator*{\argmin}{arg~min}
\DeclareMathOperator{\EE}{\mathbb{E}}
\DeclareMathOperator{\VV}{\mathbb{V}}
\DeclareMathOperator{\PP}{\mathbb{P}}
\DeclareMathOperator{\hEE}{\hat{\mathbb{E}}}
\DeclareMathOperator{\one}{\mathds{1}\hspace{-.18em}}
\DeclareMathOperator{\Reg}{{\text{Reg}}}
%\DeclareMathOperator*{\lap}{{\lessapprox}}
%\DeclareMathOperator*{\lapp}{{\lessapprox}}
\newcommand{\lap}{\mathop{}\!\lessapprox}
\newcommand{\lapp}{\mathop{}\!\lessapprox}
\newcommand{\gapp}{\mathop{}\!\gtrapprox}
\newcommand{\lsim}{\mathop{}\!\lesssim}
\newcommand{\gsim}{\mathop{}\!\gtrsim}


\def\RR{{\mathbb{R}}}
\def\NN{{\mathbb{N}}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\ubrace}[2]{{\underbrace{#1}_{\textstyle #2}}}
\newcommand{\sr}[2]{ {\stackrel{#1}{#2}} }
\newcommand*{\medcup}{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}}%
\newcommand*{\medcap}{\mathbin{\scalebox{1.5}{\ensuremath{\cap}}}}%
\def\bigmid{\,\middle|\,\xspace}
\newcommand{\fr}[2]{ { \frac{#1}{#2} }}
\newcommand{\tfr}[2]{ { \tfrac{#1}{#2} }}
\def\lt{\left}
\def\rt{\right}
\def\suchthat{\ensuremath{\mbox{ s.t. }}} 
\def\dsum{\ensuremath{\displaystyle\sum}} 
\def\der{\ensuremath{\partial}\xspace}

\def\bbeta{{{\boldsymbol \beta}}}
\def\btheta{{{\boldsymbol \theta}}}
\def\bphi{{{\boldsymbol \phi}}}
\def\barbu{{\overline{\mathbf u}}}
\def\sign{\ensuremath{\text{sign}}}
\def\hS{\ensuremath{\hat{S}}\xspace}

\def\larrow{\ensuremath{\leftarrow}\xspace} 
\def\rarrow{\ensuremath{\rightarrow}\xspace} 
\def\T{\ensuremath{\top}}  % transpose
\def\sig{\ensuremath{\sigma}\xspace}
\def\bsig{{\ensuremath{\boldsymbol{\sigma}}}}
\def\Pr{\ensuremath{\text{Pr}}} 
\def\eps{\ensuremath{\varepsilon}\xspace}
\def\diag{\ensuremath{\mbox{diag}}\xspace}
\def\supp{\ensuremath{\mbox{supp}}\xspace}
\def\decomp{\ensuremath{\mbox{decomp}}\xspace}

\def\balpha{{{\boldsymbol \alpha}}}
\def\bbeta{{{\boldsymbol \beta}}} % this causes error in section title
\def\btheta{{{\boldsymbol \theta}}} 
\def\bgamma{{{\boldsymbol \gamma}}} 
\def\hbtheta{{\widehat{\boldsymbol \theta}}} 
\def\bTheta{{{\boldsymbol \Theta}}} 
\def\bmu{{{\boldsymbol \mu}}}
\def\bpi{{\ensuremath{\bm{\pi}}\xspace}}  
\def\Dki{{\ensuremath{\Delta_{ki}}\xspace} }
\def\om{{\ensuremath{\omega}\xspace} }
\def\dt{{\ensuremath{\delta}\xspace} }
\def\sm{{\ensuremath{\setminus}\xspace} }

\def\grad{\ensuremath{\mathbf{\nabla}}\xspace}  

\def\bSigma{\ensuremath{\mathbf{\Sigma}}\xspace} 
\def\bLambda{\ensuremath{\boldsymbol{\Lambda}}\xspace} 
\def\hatbfP{\ensuremath{\widehat{\mathbf{P}}}\xspace} 
\def\hatbfpi{\ensuremath{\widehat{\boldsymbol{\pi}}}\xspace} 
\def\hatP{\ensuremath{\widehat{P}}\xspace} 
\def\hattheta{\ensuremath{\widehat{\theta}}\xspace} 
\def\hatQ{\ensuremath{\widehat{Q}}\xspace} 
\def\hatpi{\ensuremath{\widehat{\pi}}\xspace} 
\def\bftilpi{\ensuremath{\boldsymbol{\widetilde{\pi}}}\xspace} 
\def\bftilP{\ensuremath{\mathbf{\widetilde{P}}}\xspace} 
\def\bftilBeta{{\ensuremath{\boldsymbol{\widetilde{\beta}}}}\xspace} 
\def\tilpi{\ensuremath{\widetilde{\pi}}\xspace} 
\def\tilP{\ensuremath{\widetilde{P}}\xspace} 
\def\tilBeta{\ensuremath{\widetilde{\beta}}\xspace} 

\def\hatK{{\ensuremath{\widehat{K}}\xspace}} 
\def\hatT{{\ensuremath{\widehat{T}}\xspace}}
\def\hatW{{\ensuremath{\widehat{W}}\xspace}}
\def\hattau{{\ensuremath{\widehat{\tau}}\xspace}}
\def\sym{{\ensuremath{\text{Sym}}\xspace}} 

\def\logbar{{\ensuremath{\overline{\log}}}} 
\newcommand{\what}[1]{ {\ensuremath{\widehat{#1}}} }

\def\barT{\ensuremath{\overline{T}}\xspace} 
\def\bart{\ensuremath{\overline{t}}\xspace} 
\def\barV{\ensuremath{\overline{V}}\xspace} 
\def\barU{\ensuremath{\overline{U}}\xspace} 
\def\barG{\ensuremath{\overline{G}}} 
\def\barL{\ensuremath{\overline{L}}\xspace} 


\def\hatk{{\ensuremath{\what{k}}}\xspace}  
\def\ntil{\ensuremath{\tilde{n}}\xspace} 
\def\rtil{\ensuremath{\tilde{r}}\xspace} 
\def\hDelta{\ensuremath{\what{\Delta}}\xspace} 



%- ceiling and floor
\def\llfl{\left\lfloor} 
\def\rrfl{\right\rfloor}  
\def\llcl{\left\lceil}  
\def\rrcl{\right\rceil}  
\def\lfl{\lfloor} 
\def\rfl{\rfloor}  
\def\lcl{\lceil}  
\def\rcl{\rceil}  

%- pretty < and > symbol
\newcommand{\langl}{\begin{picture}(4.5,7)
\put(1.1,2.5){\rotatebox{60}{\line(1,0){5.5}}}
\put(1.1,2.5){\rotatebox{300}{\line(1,0){5.5}}}
\end{picture}}
\newcommand{\rangl}{\begin{picture}(4.5,7)
\put(.9,2.5){\rotatebox{120}{\line(1,0){5.5}}}
\put(.9,2.5){\rotatebox{240}{\line(1,0){5.5}}}
\end{picture}}

%- new on 20150826
\def\cmt{{\;//\;}}
\def\gam{{\ensuremath{\gamma}\xspace} }

%- new on 20151024
\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother

%- new on 20151123
\def\bl{{{\boldsymbol \ell}}}
\def\dsR{{{\mathds{R}}}}

%- new on 20160503
\def\cX{\ensuremath{\mathcal{X}}\xspace} 
\def\la{{\langle}}
\def\ra{{\rangle}}
\def\det{\ensuremath{\mbox{det}}}
\def\lam{\ensuremath{\lambda}}
\def\barV{\ensuremath{\overline{\mathbf{V}}}\xspace} 
\def\ibarV{\ensuremath{\overline{\mathbf{V}}^{-1}}\xspace} 
\def\iV{\ensuremath{{\mathbf{V}}^{-1}}\xspace} 
\def\hatth{\ensuremath{\widehat{\boldsymbol\theta}}\xspace} 
\def\tilth{\ensuremath{\tilde{\boldsymbol\theta}}\xspace} 
\def\barVinv{\ensuremath{\overline{\mathbf{V}}^{-1}}} 
\def\barVi{\ensuremath{\overline{\mathbf{V}}^{-1}}} 
\def\tilmu{{\ensuremath{\tilde{\mu}}\xspace} }

%- 20160705
\def\tiln{\ensuremath{\tilde{n}}\xspace} 

%- 20160728
\def\bell{{{\boldsymbol\ell}}}
\def\cC{\ensuremath{\mathcal{C}}\xspace} 
\def\cD{\ensuremath{\mathcal{D}}\xspace} 
\def\cW{\ensuremath{\mathcal{W}}\xspace} 
\def\cU{\ensuremath{\mathcal{U}}\xspace} 
\def\KL{\ensuremath{\normalfont{\mathsf{KL}}}}  

\def\l{{{\boldsymbol \ell}}}

%--- 20160829
\def\hatp{\ensuremath{\widehat p}}
\def\hatbfp{\ensuremath{\widehat{\mathbf{p}}}}
\def\tilg{\ensuremath{\widetilde{g}}}
\def\tilG{\ensuremath{\widetilde{G}}}
\def\tilbfg{\ensuremath{\widetilde{\mathbf{g}}}}
\def\bcI{\ensuremath{\boldsymbol{\mathcal{I}}}} 
\def\Active{\ensuremath{\text{Active}}}
\def\CBS{\ensuremath{\text{CBS}}}
\def\CBSE{\ensuremath{\text{CBSE}}}
\def\Regret{\ensuremath{\normalfont{\text{Regret}}}}
\def\Wealth{\ensuremath{\text{Wealth}}}
\def\CB{\ensuremath{\text{CB}}}

%--- 2016/09/16
\def\btau{\ensuremath{\boldsymbol{\tau}}\xspace} 
\newcommand{\wtil}[1]{ {\ensuremath{\widetilde{#1}}} }
\def\ccH{\ensuremath{c_\text{H}}}
\def\tH{\ensuremath{\text{H}}}
\def\bfeta{\ensuremath{\boldsymbol{\eta}}} 
\def\til{\widetilde} 
\def\vec{\text{vec}} 
\def\dsN{{{\mathds{N}}}}
\newcommand{\wbar}[1]{ {\ensuremath{\overline{#1}}} }
\def\barbeta{\wbar{\beta}}
\def\tilbeta{\tilde{\beta}}
\def\barC{\ensuremath{\wbar{C}}}
\def\tilC{\ensuremath{\wtil{C}}}
\def\barth{\ensuremath{\wbar{\boldsymbol\theta}}\xspace} 

\def\dsR{\ensuremath{{\mathds R}}\xspace}
\def\hcalX{\ensuremath{\what{\mathcal X}}\xspace}
\def\hcalZ{\ensuremath{\what{\mathcal Z}}\xspace}
%\def\hth{\ensuremath{\what{\theta}}\xspace}
\def\bth{{{\boldsymbol \theta}}} 
\def\bfeta{{{\boldsymbol \eta}}} 
\def\hbth{{\what{\boldsymbol \theta}}} 
\def\hth{{\hat{ \theta}}} 
\def\bfUp{\ensuremath{\mathbf{U}_\perp}\xspace}
\def\Up{\ensuremath{\mathbf{U}_\perp}\xspace}
\def\lam{{\ensuremath{\lambda}\xspace} }
\def\bTheta{{{\boldsymbol \Theta}}}
\def\bTh{{{\boldsymbol \Theta}}}
\def\barbV{\ensuremath{\overline{\mathbf{V}}}\xspace} 

%- 20170228
\def\tL{\ensuremath{\mathbf{\text{L}}}}
\def\vec{\ensuremath{\text{vec}}}
\def\Th{{{\boldsymbol \Theta}}} 
\def\Lam{{{{{\Lambda}}}}}
\def\bLam{{{{\boldsymbol{\Lambda}}}}}
\def\blam{{{\boldsymbol{{\lambda}}}}}
\def\bgam{{{\boldsymbol{{\gamma}}}}} 
\def\bom{{{\boldsymbol{{\omega}}}}} 
\def\lnorm{\left|\left|}
\def\rnorm{\right|\right|}

\def\hU{\ensuremath{\what{\U}}\xspace} 
\def\hV{\ensuremath{\what{\V}}\xspace} 
\def\hS{\ensuremath{\what{\S}}\xspace} 
\def\hTh{\ensuremath{\what{\Th}}\xspace} 
\def\hcX{\ensuremath{\what{\cX}}\xspace} 
\def\hcZ{\ensuremath{\what{\cZ}}\xspace} 
\def\hUp{\ensuremath{\what{\U}_\perp}} 

\def\bbP{\ensuremath{\mathbb{P}}} 
\def\Pp{\ensuremath{\mathbf{P}_\perp}} 
\def\hP{\ensuremath{\what{\mathbf{P}}}} 
\def\hPp{\ensuremath{\what{\mathbf{P}}_\perp}} 
\def\hK{\ensuremath{\what{\K}}} 
\def\Vp{\ensuremath{\mathbf{V}_\perp}\xspace}
\def\tilTh{\ensuremath{\widetilde{\boldsymbol\Theta}}\xspace} 
\def\alp{\ensuremath{{\boldsymbol\alpha}}\xspace}
\def\alpp{\ensuremath{\boldsymbol\alpha_\perp}}
\def\tilalp{\ensuremath{\widetilde{\boldsymbol\alpha}}}
\def\tilalpp{\ensuremath{\widetilde{\boldsymbol\alpha}_\perp}}
\def\halp{\ensuremath{\what{\boldsymbol\alpha}}}
\def\halpp{\ensuremath{\what{\boldsymbol\alpha}_\perp}}

\def\hy{\ensuremath{\hat{\y}}} 
%\def\bu{\ensuremath{\mathbf{u}}} 
\def\dH{\ensuremath{\normalfont{\text{d}_\text{H}}}} 
\def\Rad{\ensuremath{\text{\normalfont{Rad}}}} 
\def\tilq{\ensuremath{\widetilde{q}}} 
\def\cS{{\ensuremath{\mathcal{S}}}} 
\def\AUL{{\ensuremath{\normalfont{\text{AUL}}}}} 
\def\Rel{{\ensuremath{\normalfont{\text{Rel}}}}} 
\def\cF{{\ensuremath{\mathcal{F}}}} 
\def\Mis{{\ensuremath{\normalfont{\text{Mis}}}}} 

\def\tilell{\ensuremath{\tilde{\ell}}} 
\def\btilell{\ensuremath{\widetilde{\boldsymbol{\ell}}}} 
\def\tilL{\ensuremath{\widetilde{L}}} 
\def\barJ{\ensuremath{\overline{J}}} 

% 20171016
\def\Corral{\ensuremath{\normalfont{\textsc{Corral}}}\xspace}
\def\cO{{\ensuremath{\mathcal{O}}}} 
\def\tilO{{\ensuremath{\widetilde{\mathcal{O}}}}} 
\def\Eps{\ensuremath{\mathcal{E}}}
\def\bth{\ensuremath{{\boldsymbol{\theta}}}} 
\def\cR{\ensuremath{\mathcal{R}}} 

\def\SUCB{\ensuremath{\normalfont{\text{SUCB}}}}
\def\tr{{\ensuremath{\normalfont{\text{tr}}}}} 

\def\hcL{\ensuremath{\hat\cL}} 
\def\hS{\ensuremath{\hat S}} 
\def\hL{\ensuremath{\hat\L}} 
\def\hLam{\ensuremath{\what{\Lam}}\xspace} 

\def\dsP{\ensuremath{{\mathds P}}}

%- 20180418
\def\cK{\ensuremath{\mathcal{K}}}
\def\nab{\ensuremath{\nabla}}
\def\th{{\ensuremath{\theta}}}

\def\bPhi{{{\boldsymbol \Phi}}} 
\def\bGamma{{{\boldsymbol \Gamma}}} 




%- 20180426
\def\hVp{\ensuremath{\what{\V}_\perp}} 
\def\baru{\ensuremath{\overline{\u}}} 
\def\barv{\ensuremath{\overline{\v}}} 
\def\bbU{\ensuremath{\overline{\U}}} 
\def\bbV{\ensuremath{\overline{\V}}} 
\def\hbS{\ensuremath{\what{\S}}}

\def\sign{\ensuremath{\normalfont{\text{sign}}}} 
\def\Var{\ensuremath{\normalfont{\text{Var}}}}
\def\Om{{\ensuremath{\Omega}}} 

\def\poly{\operatorname{poly}}
\def\Misid{\operatorname{Misid}}
\def\cH{{\ensuremath{\mathcal{H}}}}
\def\hG{\ensuremath{\hat{G}}} 
\def\hg{\ensuremath{\hat{g}}} 
\def\nab{\ensuremath{\nabla}} 

\def\Reward{\ensuremath{\text{Reward}}}
\def\tiltheta{\ensuremath{\tilde{\theta}}} 
\def\tilp{\ensuremath{\tilde{p}}} 

\def\bxi{{{\boldsymbol \xi}}}
\def\bone{{{\mathbf 1}}}

\def\hell{{{\hat\ell}}}
\let\SS\undefined

\def\rhoX{{\rho_{\mathcal{X}}}}
\def\Mis{{\text{Mis}}}

%2019
\def\hR{\ensuremath{\widehat{R}}} 
\def\hcF{\ensuremath{\widehat{\cF}}} 
\def\suchthat{\text{ s.t. }}
\def\cd{\cdot}
\def\cc{{\circ}}
\def\hf{\ensuremath{\widehat{f}}} 
\def\bargam{\ensuremath{\overline{\gamma}}} 
\def\tila{\ensuremath{\widetilde{a}}} 
\def\tilmu{\ensuremath{\widetilde{\mu}}}
\def\tilf{\ensuremath{\widetilde{f}}} 
\def\tilcF{\ensuremath{\widetilde{\cF}}} 
\def\barcF{\ensuremath{\overline{\cF}}} 
\def\barf{\ensuremath{\overline{f}}} 
\def\bara{\ensuremath{\overline{a}}} 
\def\barmu{\ensuremath{\overline{\mu}}} 

\newcommand{\FSB}{{\ensuremath{\text{FSB}}}}
\newcommand{\Cr}{{\ensuremath{\text{Cr}}}}
\newcommand{\SE}{{\ensuremath{\text{SE}}}}
\def\IC{{\ensuremath{\normalfont{\text{IC}}}}}
\newcommand{\barB}{{\ensuremath{\wbar B}}}
\newcommand{\barS}{{\ensuremath{\wbar S}}}
\newcommand{\barF}{{\ensuremath{\wbar F}}}
\newcommand{\Fs}{{\ensuremath{\text{Fs}}}}
\newcommand{\barFs}{{\ensuremath{\wbar{\text{Fs}}}}}
\def\rcF{\ensuremath{\mathring{\cF}}} 
\def\rbeta{\ensuremath{\mathring{\beta}}} 
\def\Cf{{\ensuremath{{\normalfont{\text{Cf}}}}}}
\def\barCf{{\ensuremath{\wbar{\text{Cf}}}}}
\def\ralpha{\ensuremath{{\mathring{\alpha}}}} 
\newcommand{\Fb}{{\ensuremath{\text{Fb}}}}
\def\rz{\ensuremath{\mathring{z}}} 

\DeclareMathOperator{\SReg}{{\mathsf{SReg}}}
\DeclareMathOperator{\MisPrb}{{{\mathsf{MisPrb}}}}
\def\SR{{\ensuremath{\text{SR}}}\xspace}
\def\lin{{\ensuremath{\mathsf{lin}}}}
\def\Bernoulli{{\ensuremath{\mathsf{Bernoulli}}}}
\def\dtmin{{\delta_{\min}}}
\renewcommand{\vec}{{\mathsf{vec}}}
\newcommand{\F}{{\mathsf{F}}}

\def\smin{{s_{\min}}}
\newcommand\kmax[1]{\mathop{#1\hyphen\max}}
\def\hyphen{{\text{-\hspace{-.06em}}}}
\def\lammin{{\lambda_{\min}}}

\newcommand\msf[1]{{\mathsf{#1}}}

\DeclareMathOperator{\barln}{\overline\ln}%

\def\barH{\ensuremath{\bar{H}}} 

\newcommand{\myparagraph}[1]{\paragraph{[#1]}\mbox{}\\}


\def\horizontalline{\noindent\rule{\textwidth}{1pt} }
\DeclareMathOperator{\Supp}{{\mathsf{Supp}}}
\def\Approx{{\mathsf{Approx}} }
\def\ddmu{{\ddot\mu}}
\def\hlam{{\hat\lambda}}

\def\eff{{\mathsf{eff}}}
\def\Seff{{S_{\mathsf{eff}}}}
\def\opt{{\mathsf{opt}}}
\def\pes{{\mathsf{pes}}}
\def\faury{{\mathsf{faury}}}
\def\nice{{\textsf{nice} } } 


\def\dmu{\dot\mu}
\def\mc#1{\mathcal{#1}} % adjusting location of box in table
\def\teff{{\ensuremath{t_\mathsf{eff}}}}
\def\naive{{\mathsf{naive}}} 
\def\tw{\mathsf{w}}

\newcommand{\HOMER}{\texttt{HOMER}\xspace}
\newcommand{\WAR}{\texttt{WAR}\xspace}


==> mixing.tex <==
\section{Mixing different designs}

In the regret minimization algorithm, our design objective was over a maximum of two sub-objectives as in the pure exploration algorithm of \cite{jun2020improved}. One may expect that we could compute two separate designs and mix the two of them. In this section, we explore this idea.  

% Consider the following burn in objective: 
% $$ f(\lambda) :=
%         \gamma(d, |\X_k|, \delta_k)^{-1}\max_{x\in\X_k} \|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2$$
% and the design $\lambda_k^f = \arg\min_{\lambda\in\Delta_{\X}}f(\lambda)$. 
% Let $n_k^f = f(\lambda_k^f)$. 
% Additionally, consider the XY objective: 
% $$g(\lambda) :=2^{2k} 
%                 \max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda, \hat{\theta}_{0})^{-1}}^2 $$
% and the design $\lambda_k^g = \arg\min_{\lambda\in\Delta_{\X}}g(\lambda)$. 
% Let $n_k^g = g(\lambda_k^f)$. Let $\lambda_{k,i}^f$ be the fraction of samples given to arm $i$ under allocation $\lambda_k^f$, and let $\lambda_{k,i}^g$ be defined similarly. 
% Our mixed design for arm $i$ will be proportional to
% $$\Tilde{\lambda}_{k,i} := \max\left\{\frac{n_k^f}{n_k^f + n_k^g}\lambda_{k,i}^f, \frac{n_k^g}{n_k^f + n_k^g}\lambda_{k,i}^g \right\}. $$
% Note that this need not sum to 1, and we must re-normalize. Precisely, let $\lambda_{k,i} = \Tilde{\lambda}_{k,i} / \sum_j\Tilde{\lambda}_{k,j}$. Then we have that for any $\theta$,
% \begin{align*}
%     H(\lambda_k, \theta)& = \sum_{i=1}^n \lambda_{k,i}\dot{\mu}(\bx_i^T\theta)\bx_i\bx_i^T\\
%     & = \frac{1}{\sum_j\Tilde{\lambda}_{k,j}}\sum_{i=1}^n \max\left\{\frac{n_k^f}{n_k^f + n_k^g}\lambda_{k,i}^f, \frac{n_k^g}{n_k^f + n_k^g}\lambda_{k,i}^g \right\}\dot{\mu}(\bx_i^T\theta)\bx_i\bx_i^T \\
%     & \succeq \frac{1}{\sum_j\Tilde{\lambda}_{k,j}}\frac{n_k^f}{n_k^f + n_k^g}\sum_{i=1}^n \lambda_{k,i}^f \dot{\mu}(\bx_i^T\theta)\bx_i\bx_i^T\\
%     & = \frac{1}{\sum_j\Tilde{\lambda}_{k,j}}\frac{n_k^f}{n_k^f + n_k^g} H(\lambda_k^f, \theta)
% \end{align*}
% Note that
% \begin{align*}
%     \sum_{j=1}^n\Tilde{\lambda}_{k, j} & \leq \max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\} \sum_{j=1}^n\max\{\lambda_{k,j}^f, \lambda_{k,j}^g\}\\
%     & \leq \max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\} \sum_{j=1}^n\lambda_{k,j}^f +  \lambda_{k,j}^g \\
%     & = 2\max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\}. 
% \end{align*}
% Hence, 
% \begin{align*}
%     H(\lambda_k, \theta)& \succeq 
%     \frac{1}{2}\frac{\frac{n_k^f}{n_k^f + n_k^g}}{\max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\}}
%     H(\lambda_k^f, \theta) \succeq \frac{1}{2}\frac{\frac{n_k^f}{n_k^f + n_k^g}}{\frac{n_k^f}{n_k^f + n_k^g} + \frac{n_k^g}{n_k^f + n_k^g} }
%     H(\lambda_k^f, \theta)
%      = \frac{1}{2}\frac{n_k^f}{n_k^f + n_k^g}
%     H(\lambda_k^f, \theta).
% \end{align*}
% This implies that
% \begin{align*}
%      H(\lambda_k, \theta)^{-1}\preceq 2\frac{n_k^f + n_k^g}{n_k^f}H(\lambda_k^f, \theta)^{-1}.
% \end{align*}
% We have a similar relationship for $H(\lambda_k^g, \theta)$ as well.
% Then, let the number of samples in round $k$ be $n_k^f + n_k^g$ (multiplied by the appropriate log factors, but let's ignore this for brevity). 
% Applying this to the burn-in condition, we have that
% \begin{align*}
%     \max_{x\in\X_k} \|x\|_{H_{n_k}({\theta}_{\ast})^{-1}}^2 & \leq \frac{(1+\epsilon)}{n_k}\max_{x\in\X_k} \|x\|_{H(\lambda_k, {\theta}_{\ast})^{-1}}^2 \\
%     & = \frac{(1+\epsilon)}{n_k^f + n_k^g}\max_{x\in\X_k} \|x\|_{H(\lambda_k, {\theta}_{\ast})^{-1}}^2 \\
%     & \leq 2\frac{(1+\epsilon)}{n_k^f}\max_{x\in\X_k} \|x\|_{H(\lambda_k^f, {\theta}_{\ast})^{-1}}^2 \\
%     & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} \frac{3(1+\epsilon)}{n_k^f}\max_{x\in\X_k} \|x\|_{H(\lambda_k, \hat{\theta}_{k})^{-1}}^2\\
%     & \leq \gamma(d, |\X_k|, \delta_k)^{-1}.
% \end{align*}
% Hence, the mixed allocation satisfies the burn in condition need in each round. Furthermore, applying the mixed distribution to control the deviations in mean parameter space, 
% \begin{align*}
%     |\mu(\hat{\theta}_k^T\bx_s) - \mu({\theta}_\ast^T\bx_s)| &\leq 3.5e\sqrt{\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H_{n_k}(\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}\\
%     & \leq 3.5e\sqrt{\frac{(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k,\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k}}\\
%     & = 3.5e\sqrt{\frac{(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k,\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^f + n_k^g}}\\
%     %%%%%%%%%%%%
%     & \leq 3.5e\sqrt{\frac{2(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k^g,\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^g}}\\
%     %%%%%%%%%%%%%
%     & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} 3.5e\sqrt{\frac{6(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k^g,\theta_k)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^g}}\\
%     & \stackrel{\text{Lemma 5, \cite{jun2020improved}}}{\leq} 3.5e\sqrt{\frac{6e(1+\epsilon)\dot{\mu}(\bx^T\hat{\theta}_k)^2\|\bx\|_{H(\lambda_k^g,\theta_k)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^g}}\\
%     & \leq 2^{-k}
% \end{align*}
% These pieces are jointly enough to redo Lemma~\ref{lem:mean_param_regret_correct} which implies correctness. Hence, the algorithm can use this instead. 

\subsection{Algorithm}

In this section, we develop an algorithm that mixes two optimal designs-- one to ensure the burn in condition holds and another to optimally estimate the means. 

\begin{algorithm}[ht] \caption{MDMA: Mixed Designs Mean-parameter Algorithm}
    \label{alg:mix-exp-design-regret}
    \begin{algorithmic}
        \Require{$\epsilon$, $\delta$, $\X$, $\kappa_0$, rounding procedure}
        \State{$k=1, \X_1 = \X$, $\gamma(d, \S, \delta) = d + \log(6(2+|\S|)/\delta)$}
        \State {$\hat\theta_0\leftarrow$ \textbf{BurnIn}($\X, \kappa_0$)}  \Comment{Burn-in phase}
        \While{$|\X_k| > 1$ } \Comment{Elimination phase}
        % \State  $\delta_k = \delta/(2|\X|k^2)$
        \State  $\delta_k = \delta/(4(2+|\X|)|\X|k^2)$
        \State $\lambda_{k}^f = \arg\min_{\lambda\in \Delta_{\X_k}}f(\lambda)$ for  $f(\lambda) :=
               \max_{x\in\X_k} \|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2$
        \State $\lambda_{k}^g = \arg\min_{\lambda\in \Delta_{\X_k}}g(\lambda)$ for  $g(\lambda) := 
                \max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2$
        % \State$f(\lambda) :=
        %         \max\left\{2^{2k} 
        %         \max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2, \gamma(d, |\X_k|, \delta_k)^{-1}\max_{x\in\X_k} \|x\|_{H(\lambda, \hat{\theta}_{k-1})^{-1}}^2\right\}$
        \State $n_k^f =  6(1+\epsilon)\gamma(d, |\X_k|, \delta) f(\lambda_k^f)$ and  $n_k^g = 6(1+\epsilon)3.5^2 e^3 2^{2k}g(\lambda_k^g)\log(\delta_k^{-1})$. 
        \State $\lambda_k = \arg\min_{\lambda\in \Delta_{\X_k}} f(\lambda)$
        % \State{$n_k = \max\{3.5^2(1+\epsilon)\cdot e^3\cdot f(\lambda_k)\log(1/\delta_k), r(\epsilon)\}$}
        \State{Let $\Tilde{\lambda}_{k,i} := \max\left\{\frac{n_k^f}{n_k^f + n_k^g}\lambda_{k,i}^f, \frac{n_k^g}{n_k^f + n_k^g}\lambda_{k,i}^g \right\}$ 
         where $\lambda_{k,i}^f$ and $\lambda_{k,i}^g$ are the $i^\text{th}$ entry of $\lambda_k^f$ and $\lambda_k^g$}
         \State{Let $\lambda_{k,i} = \Tilde{\lambda}_{k,i} /\sum_{j=1}^n\Tilde{\lambda}_{k,j}$ and $n_k = \max\{n_k^f + n_k^g, r(\epsilon)\}$}
        \State{$x_1, \cdots x_{n_k}=\rdp(\lceil n_k\rceil, \lambda_k, \epsilon) $}
        % \State{$n_k^B =  \lceil f(\lambda_k^B)\lambda_k^B\rceil\in \Delta_{\X_k}$ and $n_k =  \lceil f(\lambda_k^B)\lambda_k\rceil\in \Delta_{\X_k}$}
        % \State{Pull each $x_i$, $n_{k,i}$ and $n_{k,i}^B$ times.} 
        \State{Observe rewards $y_1, \cdots, y_{n_k}$ and Compute the MLE $\hat\theta_k$ with $ \{(x_i,y_i)\}_{i=1}^{n_k}$. }
        % \State{$\hat{x}_k = \arg\max_{x\in\X_k} \hat\theta_k^\top x$}
        \State{$\X_{k+1}\leftarrow \X_k \setminus \left\{x\in \X_k:\max_{x'\in \X_k}\mu(x'^T\hat{\theta}_k) - \mu(x^T\hat{\theta}_k) \geq 2\cdot 2^{-k}\right\}$}
        \State{$k\gets k+1$}
		\EndWhile
	\end{algorithmic}
\end{algorithm}


\subsection{Theory}

\begin{theorem}\label{thm:mix_regret_complexity}
Fix $\delta \leq e^{-1}$ and suppose there is a generic burn in algorithm takes $T_B$ samples and satisfies the conditions of Corollary~\ref{cor:mean_param_bound}
Define $T' := T - T_B$ to be the samples and assume $T' > 0$. Define $\S_t = \{\bx \in \X: \mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx) \leq 2^{-k}\}$. 
With probability at least $1-\delta$, 
algorithm~\ref{alg:mix-exp-design-regret}, for any $\nu > 0$ obtains a regret within a constant factor of
% \begin{align*}
%     T_B + T'\nu &+ \lceil\log_2((\Delta \vee \nu)^{-1})\rceil r(\epsilon) + (1+\epsilon)\gamma(d, |\X|, \delta) \min_\lambda\max_{x\in\X} \|x\|_{H(\lambda, {\theta}_{\ast})^{-1}}^2 
%     \\ & (1+\epsilon)
%     \log\left(\frac{|\X|\lceil \log_2( (\Delta \vee \nu)^{-1})\rceil}{\delta}\right)\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil \max_{x\in\S_k} \frac{\dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2}{\Delta_x \vee \nu}
% \end{align*}
\begin{align*}
    T_B + T'\nu &+ \lceil\log_2((\Delta \vee \nu)^{-1})\rceil r(\epsilon) + (1+\epsilon)\gamma(d, |\X|, \delta) \min_\lambda\max_{x\in\X} \|x\|_{H(\lambda, {\theta}_{\ast})^{-1}}^2 
    \\ &  + (1+\epsilon)
    \log\left(\frac{|\X|\lceil \log_2( (\Delta \vee \nu)^{-1})\rceil}{\delta}\right)\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} \min_\lambda\max_{x\in\S_k} \frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x \vee \nu}
\end{align*}
Minimizing $\nu$, we achieve a minimax regret of 
\begin{align*}
    \widetilde{O}\left(\sqrt{T\min_\lambda\max_{\bx}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2\log(|X|/\delta)}  + T_B\right)
\end{align*}
Note that $T_B$ can be chosen to be $ O(d^2/\kappa)$. Additionally, setting $\nu = 0$, Algorithm \ref{alg:mix-exp-design-regret} achieves an instance dependent regret of 
\begin{align*}
    \widetilde{O}\left(\min_{\lambda \in \Delta_{\X}}\max_{\bx\in \X}\frac{\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x}\log(|X|/\delta) \right)
\end{align*}
where $\widetilde{O}$ hides constants and doubly logarithmic factors. 
\end{theorem}

\begin{remark}
Note that $\min_\lambda\max_{\bx}\dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 =\min_\lambda\max_{\bx} \dot{\mu}(x^T{\theta}_{\ast})\|\sqrt{\dot{\mu}(x^T{\theta}_{\ast})}x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 \leq d/4$ by the Kiefer-Wolfowitz Theorem, \cite{lattimore2020bandit}, Theorem 21.1. Hence the regret is bounded by $\Tilde{O}(\sqrt{dT\log(|X|/\delta)})$. However, $\dot{\mu}(x^T{\theta}_{\ast})$ can be exponentially smaller than $1/4$. 
\end{remark}


\begin{lemma}\label{lem:mix_h_vs_normal}
For any $\theta$, $H(\lambda_k, \theta)^{-1}\preceq 2\frac{n_k^f + n_k^g}{n_k^f}H(\lambda_k^f, \theta)^{-1}$ and $H(\lambda_k, \theta)^{-1}\preceq 2\frac{n_k^f + n_k^g}{n_k^g}H(\lambda_k^g, \theta)^{-1}$
\end{lemma}

\begin{proof}
For any $\theta$,
\begin{align*}
    H(\lambda_k, \theta)& = \sum_{i=1}^n \lambda_{k,i}\dot{\mu}(\bx_i^T\theta)\bx_i\bx_i^T\\
    & = \frac{1}{\sum_j\Tilde{\lambda}_{k,j}}\sum_{i=1}^n \max\left\{\frac{n_k^f}{n_k^f + n_k^g}\lambda_{k,i}^f, \frac{n_k^g}{n_k^f + n_k^g}\lambda_{k,i}^g \right\}\dot{\mu}(\bx_i^T\theta)\bx_i\bx_i^T \\
    & \succeq \frac{1}{\sum_j\Tilde{\lambda}_{k,j}}\frac{n_k^f}{n_k^f + n_k^g}\sum_{i=1}^n \lambda_{k,i}^f \dot{\mu}(\bx_i^T\theta)\bx_i\bx_i^T\\
    & = \frac{1}{\sum_j\Tilde{\lambda}_{k,j}}\frac{n_k^f}{n_k^f + n_k^g} H(\lambda_k^f, \theta)
\end{align*}
Note that
\begin{align*}
    \sum_{j=1}^n\Tilde{\lambda}_{k, j} & \leq \max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\} \sum_{j=1}^n\max\{\lambda_{k,j}^f, \lambda_{k,j}^g\}\\
    & \leq \max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\} \sum_{j=1}^n\lambda_{k,j}^f +  \lambda_{k,j}^g \\
    & = 2\max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\}. 
\end{align*}
Hence, 
\begin{align*}
    H(\lambda_k, \theta)& \succeq 
    \frac{1}{2}\frac{\frac{n_k^f}{n_k^f + n_k^g}}{\max\left\{\frac{n_k^f}{n_k^f + n_k^g}, \frac{n_k^g}{n_k^f + n_k^g} \right\}}
    H(\lambda_k^f, \theta) \succeq \frac{1}{2}\frac{\frac{n_k^f}{n_k^f + n_k^g}}{\frac{n_k^f}{n_k^f + n_k^g} + \frac{n_k^g}{n_k^f + n_k^g} }
    H(\lambda_k^f, \theta)
     = \frac{1}{2}\frac{n_k^f}{n_k^f + n_k^g}
    H(\lambda_k^f, \theta).
\end{align*}
This implies that
\begin{align*}
     H(\lambda_k, \theta)^{-1}\preceq 2\frac{n_k^f + n_k^g}{n_k^f}H(\lambda_k^f, \theta)^{-1}.
\end{align*}
The proof for $H(\lambda_k^g, \theta)$ follows identically.
\end{proof}



\begin{lemma}\label{lem:mix_mean_param_regret_correct}
For any $\delta \leq e^{-1}$, with probability at least $1-\delta$, for all rounds $k\in \N$ we have that $\bx_\ast \in \X_k$ and $\max_{\bx\in \X_k}\mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx) \leq 8\cdot 2^{-k}$. 
\end{lemma}

\begin{proof}
First note that
\begin{align*}
    \max_{x\in\X_k} \|x\|_{H_{n_k}({\theta}_{\ast})^{-1}}^2 & \leq \frac{(1+\epsilon)}{n_k}\max_{x\in\X_k} \|x\|_{H(\lambda_k, {\theta}_{\ast})^{-1}}^2 \\
    & = \frac{(1+\epsilon)}{n_k^f + n_k^g}\max_{x\in\X_k} \|x\|_{H(\lambda_k, {\theta}_{\ast})^{-1}}^2 \\
    & \stackrel{\text{Lemma}~\ref{lem:mix_h_vs_normal}}{\leq} 2\frac{(1+\epsilon)}{n_k^f}\max_{x\in\X_k} \|x\|_{H(\lambda_k^f, {\theta}_{\ast})^{-1}}^2 \\
    & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} \frac{6(1+\epsilon)}{n_k^f}\max_{x\in\X_k} \|x\|_{H(\lambda_k, \hat{\theta}_{k})^{-1}}^2\\
    & \leq \gamma(d, |\X_k|, \delta)^{-1}.
\end{align*}
Hence, the mixed allocation satisfies the burn in condition need in each round.
Furthermore, by Corollary~\ref{cor:mean_param_bound}, and Lemma~\ref{lem:burnin_guarantee},
we have that with probability $1-\delta_k$,
\begin{align*}
    |\mu(\hat{\theta}_k^T\bx_s) - \mu({\theta}_\ast^T\bx_s)| &\leq 3.5e\sqrt{\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H_{n_k}(\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}\\
    & \leq 3.5e\sqrt{\frac{(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k,\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k}}\\
    & = 3.5e\sqrt{\frac{(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k,\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^f + n_k^g}}\\
    %%%%%%%%%%%%
    & \leq 3.5e\sqrt{\frac{2(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k^g,\theta_\ast)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^g}}\\
    %%%%%%%%%%%%%
    & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} 3.5e\sqrt{\frac{6(1+\epsilon)\dot{\mu}(\bx^T\theta_\ast)^2\|\bx\|_{H(\lambda_k^g,\theta_k)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^g}}\\
    & \stackrel{\text{Lemma 5, \cite{jun2020improved}}}{\leq} 3.5e\sqrt{\frac{6e(1+\epsilon)\dot{\mu}(\bx^T\hat{\theta}_k)^2\|\bx\|_{H(\lambda_k^g,\theta_k)^{-1}}^2 \log(2(2+|\X|)|\X|/\delta_k)}{n_k^g}}\\
    & \leq 2^{-k}
\end{align*}
for all $\bx \in \X_k$. Via a union bound over the rounds, this condition holds in every round. 
First, we show that the best arm, $\bx_\ast$ is never eliminated. We have that $\X_1 = \X$. Assume the inductive hypothesis that $\bx_\ast \in \X_k$. For any $\bx \in \in \X_k$,
\begin{align*}
    \mu(\htheta_k^T\bx) - \mu(\htheta_k^T\bx_\ast) 
    & = \mu(\htheta_k^T\bx) - \mu(\theta_\ast^T\bx) + \mu(\theta_\ast^T\bx) - \mu(\theta_\ast^T\bx_\ast) + \mu(\theta_\ast^T\bx_\ast) -\mu(\htheta_k^T\bx_\ast) \\
    & \leq \mu(\htheta_k^T\bx) - \mu(\theta_\ast^T\bx) + \mu(\theta_\ast^T\bx_\ast) -\mu(\htheta_k^T\bx_\ast) \\
    & \leq 2\cdot 2^{-k}.
\end{align*}
Hence, $\bx_\ast \in \X_{k+1}$. Next, we show that for any $\bx$ such that $\mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx) > 4\cdot 2^{-k}$, $\bx \not\in \X_{k+1}$. 
\begin{align*}
    \mu(\htheta_k^T\bx_\ast) - \mu(\htheta_\ast^T\bx)
    & = \mu(\htheta_k^T\bx_\ast)- \mu(\theta_\ast^T\bx_\ast) + \mu(\theta_\ast^T\bx_\ast) -  \mu(\theta_\ast^T\bx) + \mu(\theta_\ast^T\bx)  -\mu(\htheta_\ast^T\bx) \\
    & > 2\cdot 2^{-k}
\end{align*}
which implies that $\bx \not\in \X_{k+1}$. Taken together, these statements implies that the regret of any arm present in round $k$ is at most $8\cdot 2^{-k}$. 
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:mix_regret_complexity}]
% Let $T' := T - \lceil3(1+\epsilon)d\gamma(d)\log(2(2 + |\X|)|\X|/\delta)\rceil$ 
$T' = T - T_B$. 
be the number of samples taken after the burn in procedure. We assume $T' > 0$. Since all rewards are bounded by $1$, the burn in contributes at most
$T_B$. 
% $\lceil3(1+\epsilon)d\gamma(d)\log(2(2 + |\X|)|\X|/\delta)\rceil$ 
to the total regret. We proceed by bounding the remaining $T'$ samples following burn in. Let $n_k^i$ denote the number of times $\bx_i$ is pulled in round $k$ and let $\lambda_k^i$ denote the fraction of the allocation placed on arm $i$. Assume that the event in Lemma~\ref{lem:mix_mean_param_regret_correct} occurs. 
\begin{align*}
    R_{T'} & = \sum_{x \in \X \backslash \{x^\ast\}} \Delta_x T_x \\
    %%%%%%%%%%%%%%
    & \leq T'\nu + \sum_{k=1}^\infty \sum_{x \in \X \backslash \{x^\ast\}: \Delta_x > \nu} \Delta_x n_k^i \\
    %%%%%%%%%%%%%%
    & \stackrel{\text{rounding}}{\leq} T'\nu + \lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil r(\epsilon) + \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} \sum_{x \in \X \backslash \{x^\ast\}: \Delta_x > \nu} \Delta_x n_k\lambda_k^i \\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu +\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil r(\epsilon) + 8\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} \lceil n_k\rceil \\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu + 2\log_2(8 (\Delta \vee \nu)^{-1}) r(\epsilon) + 8\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} n_k \\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu + 2\lceil\log_2(8 (\Delta \vee \nu)^{-1})\rceil  r(\epsilon) + 8\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} n_k \\
    %%%%%%%%%%%%%%%%%%
    & \leq T'\nu + 2\lceil\log_2(8 (\Delta \vee \nu)^{-1})\rceil  r(\epsilon)+ \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}8\cdot 2^{-k} n_k^f  + \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 8\cdot2^{-k} n_k^g
\end{align*}
We analyze each sum individually. 
\begin{align*}
    \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} n_k^f 
    & = 6(1+\epsilon)\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k}\gamma(d, |\X_k|, \delta) f(\lambda_k^f) \\
    & \leq 6(1+\epsilon)\gamma(d, |\X|, \delta)\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} \max_{x\in\X_k} \|x\|_{H(\lambda_k^f, \hat{\theta}_{k-1})^{-1}}^2 \\
    & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} 18(1+\epsilon)\gamma(d, |\X|, \delta)\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} \max_{x\in\X_k} \|x\|_{H(\lambda_k^f, {\theta}_\ast)^{-1}}^2 \\
    & \leq 18(1+\epsilon)\gamma(d, |\X|, \delta) \min_\lambda\max_{x\in\X} \|x\|_{H(\lambda, {\theta}_{\ast})^{-1}}^2
\end{align*}
Next, 
\begin{align*}
    \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{-k} n_k^g
    & = 6(1+\epsilon)3.5^2 e^3\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}  2^{k}g(\lambda_k^g)\log(\delta_k^{-1})\\
    & = 6(1+\epsilon)3.5^2 e^3\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}  2^{k}\max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda_k^g, \hat{\theta}_{k-1})^{-1}}^2\log(\delta_k^{-1})\\
    & \stackrel{\text{Lemma 6, \cite{jun2020improved}}}{\leq} 18(1+\epsilon)3.5^2 e^3\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}  2^{k}\max_{x\in\X_k} \dot{\mu}(x^T\hat{\theta}_{k-1})^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2\log(\delta_k^{-1})\\
    & \stackrel{\text{Lemma 5, \cite{jun2020improved}}}{\leq} 18(1+\epsilon)3.5^2 e^4\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}  2^{k}\max_{x\in\X_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2\log(\delta_k^{-1})
\end{align*}
By Lemma~\ref{lem:mix_mean_param_regret_correct}, $\X_k \subset \{\bx \in \X: \mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx) \leq 8 \cdot 2^{-k}\} =: \S_k$. Therefore, the above is bounded by
\begin{align*}
    18&(1+\epsilon)3.5^2 e^3\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}  2^{k}\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2\log(\delta_k^{-1}) \\
    & \leq 18(1+\epsilon)3.5^2 e^3
    \log\left(\frac{4(2+|\X|)|\X|\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil^2}{\delta}\right)
    \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}  2^{k}\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2
\end{align*}
Finally, we have that 
\begin{align*}
    \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} & 2^{k}\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2 \\
    & \leq \lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil \max_{k \leq \lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil}2^{k}\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_\ast)^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2 \\
    & \leq \lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil \max_{x\in\S_k} \frac{\dot{\mu}(x^T{\theta}_\ast)^2\|x\|_{H(\lambda_k^g, {\theta}_\ast)^{-1}}^2}{\Delta_x \vee \nu}
\end{align*}
where the final step follows by the definition of $\S_k$. Plugging this and the previous bound back in completes the proof for a sufficiently large constant.
Furthermore, note that 
\begin{align*}
    \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} & 2^{k}\min_\lambda\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_\ast)^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 \leq \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} & \min_\lambda\max_{x\in\S_k} \frac{\dot{\mu}(x^T{\theta}_\ast)^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2}{\Delta_x \vee \nu}
\end{align*}
where we have used the definition of $\lambda_k^g$. 
\end{proof}

\newpage

\subsection{Comparison to Theorem 1 of \cite{abeille2021instance}}

\begin{remark}
The regret of the mean parameter minimization algorithm may be bounded by 
\begin{align*}
    O\left(\sqrt{dT\dot\mu^\ast\log(|\X|/\delta)}\right)
\end{align*}
up to constants and logarithmic factors. This improves over Theorem 1 of \cite{abeille2021instance} by a factor of $\sqrt{dS^2}$. 
\end{remark}

\cite{abeille2021instance} Achieve a bound of $\widetilde{O}\left(d\sqrt{T\dot\mu^\ast S^2}\right)$
up to lower order terms where $\dot\mu^\ast := \dot\mu(\theta_\ast^T\bx_\ast)$, the derivative of the mean of the best arm and $\|\theta_\ast\| \leq S$. In this section, we bound the term
\begin{align*}
    2^{k}\min_\lambda\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2
\end{align*}
which is the main complexity term in the $k^\text{th}$ round. First, we have that
\begin{align*}
    2^{k}\min_\lambda\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 
    & \leq 2^{k}\min_\lambda\max_{x\in\S_k} \left\|\sqrt{\dot{\mu}(x^T{\theta}_{\ast})}x\right\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 \cdot \max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast}) \\
    &\leq 2^{k}d \max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast}) 
\end{align*}
where the final inequality follows by the Kiefer-Wolfowitz Theorem, Thm 20.1 \cite{lattimore2020bandit}. Recall that $\S_k = \{\bx \in \X: \mu(\theta_\ast^T\bx_\ast) - \mu(\theta_\ast^T\bx) \leq 8 \cdot 2^{-k}\}$. Let $\mu^\ast := \mu(\theta_\ast^T\bx_\ast)$. 
Hence, 
\begin{align*}
    \max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast}) 
    & = \max_{x\in\S_k} \mu(x^T{\theta}_{\ast}) (1 - \mu(x^T{\theta}_{\ast})) \\
    & \leq \max_{x\in\S_k} \mu^\ast (1 - \mu(x^T{\theta}_{\ast})) \\
    & \leq \mu^\ast (1 - \mu^\ast) + 8\mu^\ast2^{-k} \\
    & \leq \dot\mu^\ast + 8\cdot2^{-k}.
\end{align*}
Plugging this in, we have that
\begin{align*}
    2^{k}\min_\lambda\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 
    \leq 2^{k}d \dot\mu^\ast + 8d.
\end{align*}
Summing this up over all rounds, we observe that 
\begin{align*}
    \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{k}\min_\lambda\max_{x\in\S_k} \dot{\mu}(x^T{\theta}_{\ast})^2\|x\|_{H(\lambda, {\theta}_\ast)^{-1}}^2 
    & \leq  \sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{k}d \dot\mu^\ast + 8d \\
    & = 8d\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil + d \dot\mu^\ast\sum_{k=1}^{\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil} 2^{k} \\
    & \leq 8d\lceil \log_2(8 (\Delta \vee \nu)^{-1})\rceil + 16d \dot\mu^\ast \nu^{-1}
\end{align*}
Note that for the rounding procedure, we necessarily have that $r(\epsilon) = \Omega(d)$. 
Hence, we may bound the regret of our algorithm up to constants and doubly logarithmic terms as
\begin{align*}
    T_B + T'\nu + \log_2((\Delta \vee \nu)^{-1}) r(\epsilon) + (1+\epsilon)d\gamma(d, |\X|, \delta) 
    +  (1+\epsilon)
    \log\left(|\X|/\delta\right)d \dot\mu^\ast \nu^{-1}
\end{align*}
for any $\nu \geq 0$. 
Choosing $\nu = O\left(\sqrt{\frac{\log\left(|\X|/\delta\right)d \dot\mu^\ast}{T}}\right)$, we observe that our regret is bounded as 
\begin{align*}
    O\left(\sqrt{dT\dot\mu^\ast\log(|\X|/\delta)}\right)
\end{align*}
which improves on the result of \cite{abeille2021instance} by a factor of $O(S\sqrt{d})$. 

==> storage.tex <==
%%%%%%%%%% Old lower bound proof %%%%%%%%%%%%%%%
% \begin{proof}
% Fix an instance $\{A, \theta\}$ and let $a(\theta)$ denote the best arm (which is random in the choice of instance). 
% Assume that there exists a $\delta_1$-PAC algorithm $\A$ that returns $a(\theta)$ and satisfies $$\E_{\theta \in \Theta}\E_{\{A, \theta\}}[T_{\delta_1}] \leq \frac{n}{2}.$$
% Fix an arbitrary sequence of actions selected by $\A$ and associated rewards: 
% $$\left\{\left(a_{(1)}, R_{(1)}\right), \cdots, \left(a_{(T_{\delta_1})}, R_{(T_{\delta_1})}\right)\right\} $$
% where $T_{\delta_1}$ is the final round after which $\A$ terminates. Towards a contradiction, assume that $T_{\delta_1} \leq n/2$. We show that this implies $\A$ suffers constant probability of error. Hence $\A$ must draw at least $n/2$ samples in expectation.

% \textbf{Step 1: $\A$ must observe a $1$ or use more than $n/2$ samples}

% Assume for contradiction that $R_{(1)} = \cdots = R_{(T_{\delta_1})} = 0$ and $T_{\delta_1} \leq n/2$. We begin by showing that this implies $\A$ makes a mistake with constant probability. 

% Since 
% $$\E_{\theta \in \Theta}\E_{\{A, \theta\}}[T_{\delta_1}] \leq \frac{n}{2}$$
% by assumption, for any instance $\{A, \theta\}$, there exists a suboptimal arm $a_i \neq a(\theta)$ such that 
% $\E[T_i] \leq 1/2$ where $T_i$ is the random variable of the number of samples of arm $i$. Let $\P_{\{A, \theta\}}(\cdot)$ and $\E_{\{A, \theta\}}[\cdot]$ denote probability and expectation under instance $\{A, \theta\}$. We have that 
% \begin{align*}
%     1/2 & \geq \E_{\{A, \theta\}}[T_i] \\
%     & = \E_{\{A, \theta\}}E[T_i | T_i > 0]\P_{\{A, \theta\}}(T_i > 0) +  \E_{\{A, \theta\}}(E^c)[T_i | T_i = 0]\P_{\{A, \theta\}}(T_i = 0) \\
%     & = \E_{\{A, \theta\}}[T_i | T_i > 0]\P_{\{A, \theta\}}(T_i > 0)\\
%     &\geq \P_{\{A, \theta\}}(T_i > 0)
% \end{align*}
% where the final inequality holds since $T_i \in \integers$. Define the event 
% $$E = \{\A \text{ returns }a(\theta)\} \cap \{T_i = 0\}.$$

% $$E = \{\A \text{ returns }a(\theta)\} \cap \{T_i = 0\}\cap\{T_{\delta} \leq n/4\}\cap \{R_1=R_2=\cdots=R_{T_{\delta_1}}=0\}.$$
% Assume $\E[T_{\delta}]\leq n/8$.
% \[\P(T_{\delta} > n/2)\leq \frac{\E[T_{\delta}]}{n/4}\leq \frac{n/8}{n/2} = 1/4\]
% \[\P(E^c) \leq \delta_1+1/8+1/4+(1-\delta_2)^{n/4}\]

% We have that
% $$\P_{\{A, \theta\}}(E^c) \leq \P_{\{A, \theta\}}(\A \text{ returns }a(\theta)) + \P_{\{A, \theta\}}(T_i = 0) \leq \delta_1 + 1/2.$$
% Therefore, $\P_{\{A, \theta\}}(E) \geq \frac{1}{2} - \delta_1$. 
% Recall from the theorem statement, that under instance $\{A, \theta_i\}$, $a(\theta_i) = a_i$ is the best arm. 
% Using the change of measure identity, (cf. Lemma 18 from \cite{kaufmann2016complexity}), we see that 
% \begin{align}\label{eq:lower_bound_change_meas}
%     \P_{\{\A, \theta_i \}}(\A \text{ returns } a(\theta)) \geq \P_{\{\A, \theta_i \}}(E) = \E_{\{\A, \theta \}}\left[\1(E)\exp(-\widehat{KL}) \right]
% \end{align}
% where 
% $$\widehat{KL} =  \sum_{i=1}^{T_{\delta_1}}\sum_{a\in A} \1[a = a_{(i)}]\left[R_{(i)}\log\left(\frac{\mu(\theta^Ta)}{\mu(\theta_i^Ta)} \right) + (1 - R_{(i)})\log\left(\frac{1 - \mu(\theta^Ta)}{1-\mu(\theta_i^Ta)} \right)\right]$$
% Recall that we have assumed in the theorem that $1-\delta_2 \leq 1-\mu(\theta_i^Ta_j) \leq 1-\delta_3 $ for all $j \in [n]$ not equal to the $i$ we have chosen. We have further assumed by contradiction that $T_{\delta_1} \leq {n/2}$ and $R_{(1)} = \cdots = R_{(T_{\delta_1})} = 0$. Furthermore, on the event $E$, we have that $T_i = 0$. Hence, the above simplifies to 
% \begin{align*}
%     \sum_{i=1}^{T_{\delta_1}}\sum_{a\in A} \1[a = a_{(i)}] \left[\log\left(\frac{1 - \mu(\theta^Ta)}{1-\mu(\theta_i^Ta)} \right)\right] 
%     \leq T_{\delta_1}\log\left(\frac{1 - \delta_3}{1-\delta_2} \right) 
%     \leq \frac{n}{2}\log\left(\frac{1 - \delta_3}{1-\delta_2} \right)
% \end{align*}
% Plugging this in to equation \eqref{eq:lower_bound_change_meas}, we see that \begin{align*}
% \P_{\{\A, \theta_i \}}(\A \text{ returns } a(\theta)) & \geq \left(\frac{1 - \delta_2}{1-\delta_3} \right)^{(n/2)}\E_{\{\A, \theta \}}\left[\1(E) \right] \\
% & = \left(\frac{1 - \delta_2}{1-\delta_3} \right)^{(n/2)}\P_{\{\A, \theta \}}(E) \\
% & \geq \left(\frac{1 - \delta_2}{1-\delta_3} \right)^{(n/2)}(1/2 - \delta_1) \\
% &> \frac{1}{25} > \delta_1.
% \end{align*}
% where the final inequality holds for $\delta_1 < 1/25$, $\delta_2 < 1 - \left(\frac{1}{625} \right)^{1/n}$, and $\delta_3 > (1-\left(\frac{1}{9} \right)^{1/n}$ as chosen in the theorem.
% Note that on the instance $\{A, \theta_i\}$, returning the arm $a(\theta)$ is an error event since $\theta_i$ was chosen to be unequal to $\theta$. The above argument can be repeated for any instance $\{A, \theta_j\}, \ j\in [n]$. This implies that if $R_{(1)} = \cdots = R_{(T_{\delta_1})} = 0$ and $T_{\delta_1} \leq n/2$, then $\A$ makes a mistake with a constant probability which is a contradiction. Therefore, we have proven that either $T_{\delta_1} > n/2$ or $\exists i \in [T_{\delta_1}]: R_{(i)} = 1$. 

% \textbf{Step 2: Observing a 1 by pulling suboptimal arms is unlikely}

% The previous step implies that either $\exists i \in [T_{\delta_1}]: R_{(i)} = 1$ or $T_{\delta_1} > n/2$. Assume for contradiction that $T_{\delta_1} \leq n/2$ and $T_{a(\theta)} = 0$, the case that the algorithm $\A$ never pulls the best arm, but observes a $1$ and uses fewer than $n/2$ samples. 

% Recall from the theorem statement that we have assumed that $\mu(\theta^Ta) \leq \delta_2$ for all $a \neq a(\theta)$. If $\A$ never pulls $a(\theta)$ for any instance $\{A, \theta\}$, then
% \begin{align*}
%     \P_{\{A, \theta\}}\left(\not\exists i \in [T_{\delta_1}]: R_{(i)} = 1 \right) & = \P_{\{A, \theta\}}\left(R_{(1)} = \cdots = R_{(T_{\delta_1})} = 0 \right) \\
%     &\geq (1-\delta_2)^{T_{\delta_1}}\\
%     &\geq (1-\delta_2)^{n/2} \\
%     &> 1/25 > \delta_1.
% \end{align*}
% The penultimate inequality holds for $\delta_1 < 1/25$ and $\delta_2 < 1 - \left(\frac{1}{625}\right)^{1/n}$ as chosen in the theorem. In particular, this shows that the probability of observing a $1$ while never pulling the best arm is less than $\delta_1$. Since $\A$ fails with constant probability if a $1$ is not observed and $T_{\delta_1} \leq n/2$, this contradicts the assumption that $T_{\delta_1} \leq n/2$ and $T_{a(\theta)} = 0$. Hence, either $T_{\delta_1} > n/2$ or $\A$ must pull the best arm so $T_{a(\theta)} \geq 1$. 

% \textbf{Step 3: Finding the best arm is unlikely}
% Recall that we have considered an arbitrary action sequence $a_{(1)}, \cdots, a_{(T_{\delta_1})} \in A$. The previous steps imply that if $T_{\delta_1} \leq n/2$ then $T_{a(\theta)} \geq 1$. Here, we consider the randomness in the possible instances. 
% $$P_{\theta \sim \text{Unif}(\Theta)}\left(T_{a(\theta)}=0 |a_{(1)}, \cdots, a_{(T_{\delta_1})}\right) \geq \left(1 - \frac{T_{\delta_1}}{n} \right) \geq 1/2 > \delta_1$$
% where the final step follows from $T_{\delta_1} \leq n/2$ by assumption. Hence, the probability that the best arm is in the first $n/2$ pulls for any action sequence is at most $1/2$. On the event that $T_{a(\theta)} = 0$ which happens with probability at least $1/2$, either $T_{\delta_1} > n/2$ or $\A$ makes a mistake with constant probability. Hence, $\A$ requires at least $n/2$ samples in expectation if it makes a mistake with probability at most $\delta_1$. 
% \end{proof}

==> updated_burnin.tex <==
\section{Updated methods for burn in}

In this section, we sketch an approach for a less pessimistic approach to burning in. The idea of this approach is that even though we do not know $\theta^\ast$, if we have that $\|\theta_\ast\| \leq r$, then we can plan for the worst case $\theta$ in that ball. Note that knowing $\kappa$ versus knowing this norm are equivalent. For compactness, let $\B_r^d := \{
\theta \in \R^d: \|\theta\| \leq \beta\}$ be the $l2$ ball of radius $r$ in $\R^d$.

\begin{algorithm}[htb]
\caption{BurnIn-v2}
	\begin{algorithmic}
        \Require $\X, \kappa_0, \epsilon, r$
		\State $\lambda_0 = \arg\min_{\lambda\in \Delta_{\X}}\max_{\theta \in \B_r^d}\max_{x\in \mathcal{X}} \|x\|_{H(\lambda, \theta)^{-1}}^{2}$ 
% 		\State $n_0 = 3\kappa_0^{-1}\gamma^{-1}\log(|\X|/\delta)$
		\State{$n_0 =  (1+\epsilon)\gamma(d)\log(2(2 + |\X|)|\X|/\delta)\min_{\lambda\in \Delta_{\X}}\max_{\theta \in \B_r^d}\max_{x\in \mathcal{X}} \|x\|_{H(\lambda, \theta)^{-1}}^{2} $}
		\State $x_1, \cdots, x_{n_0}\leftarrow \rdp(\lceil n_0\rceil, \lambda_0, \epsilon)$
        \State Pull each $x_i$, $n_{0,i}$ times and observe associated rewards $y_1, \cdots, y_{n_0}$.
		\State \Return MLE $\hat{\theta}_0$
	\end{algorithmic}
\end{algorithm}

\begin{lemma}
Fix $\delta \leq e^{-1}$. With probability at least $1-\delta$, we have that for all $\bx \in \X$, $|\bx^T(\htheta_0 - \theta_\ast)| \leq 1$ and for any $\lambda \in \Delta_{\X}$ $\frac{1}{3}H(\lambda, \theta_\ast) \leq H(\lambda, \htheta_0) \leq 3H(\lambda, \theta_\ast)$. 
\end{lemma}

\begin{proof}
First, note that for any $\lambda\in \Delta_{\X}$
\begin{align*}
\max_{\bx\in \X}\|\bx\|_{H(\lambda, \theta_\ast)^{-1}}^2 \leq  \max_{\theta \in \in \B_r^d}\max_{\bx\in \X}\|\bx\|_{H(\lambda, \theta)^{-1}}^2.
\end{align*}
Let $H_0(\theta_\ast) := \max_{s=1}^{n_0}\dot{\mu}(\bx_s^T\theta_\ast)\bx_s\bx_s^T$. At the end of the phase, we have that 
\begin{align*}
    \max_{\bx \in \X}\|\bx\|_{H_0(\theta_\ast)^{-1}}^2 
    & \leq \frac{1 + \epsilon}{n_0}\max_{\bx \in \X}\|\bx\|_{H(\lambda, \theta_\ast)^{-1}}^2\\
    & \leq \frac{1 + \epsilon}{n_0}\max_{\theta \in \in \B_r^d}\max_{\bx \in \X}\|\bx\|_{H(\lambda, \theta)^{-1}}^2\\
    & \leq \frac{1}{\gamma(d)\log(2(2 + |\X|)|\X|/\delta)}.
\end{align*}
Then, via Theorem 1 of \cite{jun2020improved}, we have for all $\bx \in \X$
\begin{align*}
|\bx^T(\htheta_0 - \theta_\ast)| & \leq 3.5\sqrt{\|\bx\|_{H_0(\theta_\ast)^{-1}}^2 \log(2(2 + |\X|)|\X|/\delta))} \\
&\leq 3,5 \sqrt{\frac{\log(2(2 + |\X|)|\X|/\delta))}{\gamma(d)\log(2(2 + |\X|)|\X|/\delta)}} \\
& \leq 1.
\end{align*}
Then, by Lemma 14 of \cite{jun2020improved}, we have that for any $\lambda \in \Delta_{\X}$
\begin{align*}
    \frac{1}{3}H(\lambda, \theta_\ast) \leq H(\lambda, \htheta_0) \leq 3H(\lambda, \theta_\ast).
\end{align*}
\end{proof}
